Sampling over Union of Joins

Data scientists often draw on multiple relational data sources for analysis. A standard assumption in learning and approximate query answering is that the data is a uniform and independent sample of the underlying distribution. To avoid the cost of join and union, given a set of joins, we study the problem of obtaining a random sample from the union of joins without performing the full join and union. We present a general framework for random sampling over the set union of chain, acyclic, and cyclic joins, with sample uniformity and independence guarantees. We study the novel problem of the union of joins size evaluation and propose two approximation methods based on histograms of columns and random walks on data. We propose an online union sampling framework that initializes with cheap-to-calculate parameter approximations and refines them on the fly during sampling. We evaluate our framework on workloads from the TPC-H benchmark and explore the trade-off of the accuracy of union approximation and sampling efficiency.

==> abstract.tex <==
\begin{abstract}
Data scientists often draw on multiple relational  data sources to collect training data. A standard assumption in machine learning is that training data is an i.i.d sample of the underlying distribution.  Given a set of joins, we consider the problem of obtaining a random sample from the union of joins without performing the full join and union. 
We present a general framework for random sampling over the  set and disjoint union of chain, acyclic, and cyclic joins, with sample uniformity and independence guarantees. We study the novel problem of union size approximation of joins and propose a direct way and an online aggregation  way of approximating the overlap size of joins. 
We evaluate our framework on workloads from the TPC-H benchmark and explore the trade-off of the accuracy of union approximation  and sampling efficiency. 
\end{abstract}

==> algorithm-bkup.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|p{0.7\linewidth}}
    \hline
    $J_j$ & chain join path $J_j = R_{j,1} \bowtie_{A_{j,1}} R_{j,2} \bowtie_{A_{j,2}} \cdots \bowtie_{A_{j,n_1-1}} R_{j,n_1}$\\
    \hline
    $R_{j,i}$ & relation $i$ in join path $J_j$\\
    \hline
    $A_{j,i}$ & set of attributes
    $R_{j,i}$ and $R_{j,i+1}$ join on in $J_j$\\
    \hline
    $S$ & set of join paths $S = \{J_1,\dots,J_n\}$\\
    \hline
    $V$ & disjoint union of join paths $V = J_1\sqcup\ldots\sqcup J_n$\\
    \hline
    $U$ & set union of join paths $U = J_1\cup\ldots\cup J_n$\\
    \hline
    $\mathcal{A}_j^k$ & set of tuples of $k$-th overlapped in $J_j$\\
    \hline
    $\Delta_k$ & subset of joins of $S$ where $|\Delta_k| = k$\\
    \hline
    $\mathcal{O}_{\Delta_k}^k$ & set of overlap tuples of joins in set $\Delta_k$\\
    \hline
     $\mathcal{C}_A(R_i)$ & set of values of attribute $A$ in $R_i$\\
     \hline
     $c_A(R_i)$    & cardinality of attribute $A$ in $R_i$\\
     \hline
     $d_A(v,R_i)$  &  degree of value $v$ in $R_i$ on attribute $A$\\
     \hline
     $M_A(R_i)$ & maximum degree of values in $R_i$ on attribute $A$\\
     \hline
     $\mathcal{N}_j(i)$ & upper bound of number of tuples after the $i$th join in $J_j$\\
     \hline
     $\mathcal{N}_j(v, i)$ & upper bound of number of tuples with $v$ on $A_{i,1}$ after the $i$th join in $J_j$\\
     \hline
     $\mathcal{K}(i)$  & upper bound of number of overlapping tuples after the $i$th join in join paths\\
     \hline
     $\mathcal{K}(v, i)$ & upper bound of number of overlapping tuples with $v$ on $A_{i,1}$ after the $i$th join in join paths\\
     \hline
    \end{tabular}
    \caption{Notations}
    \label{tab:notations}
\end{table}

% \subsection{Old version}
% $P(J_i) = \frac{\sum_{k=1}^n\frac{1}{k}A_i^k}{|J_1\cup\cdots\cup J_n|}$, where $A_{i}^k$ is the number of the tuples of $k$-th overlapped. %(TODO: Needs to calculate $A_i^k$)
% \\
% The acceptance rate is $ \frac{|J_i| }{\sum_{k=1}^n\frac{1}{k}A_i^k }$
% \\ \textit{Remark: $A_i^k$ is a non-trival information, there should be equations to compute it. We leave a Theorem for it.}\\
% \textit{Show $\sum_{i=1}^n P(J_i) = 1$.}


% \subsection{Bounds}
% For the upper bound, we let $O_{ik}$ be the pairwise overlapping between $J_i$ and $J_k$. And we further define $O_{ii}=0$. It is easy to see that  $A_i^1+\frac{1}{2}\sum_{k} O_{ik} \geq \sum_{k=1}^n\frac{1}{k}A_i^k $.
% Then we use $\widetilde{P(J_i)}= \frac{A_i^1+\frac{1}{2}\sum_{k} O_{ik}}{|J_1\cup\cdots\cup J_n|}$. \\
% The acceptance rate is $ \frac{|J_i| }{A_i^1+\frac{1}{2}\sum_{k} O_{ik} }$.\\
% \textcolor{blue}{However, the probability above is not a valid distribution. We may revise it to be normalised: $\widetilde{P(J_i)}= \frac{2A_i^1+\sum_{k} O_{ik}}{ 2\sum_i A_i^1 +\sum_{i} \sum_{k} O_{ik}}$.\\
% The acceptance rate is $ \frac{|J_i| \cdot ( 2\sum_i A_i^1 +\sum_{i} \sum_{k} O_{ik})}{C \cdot (\sum_{k} O_{ik}+2A_i^1)}$.\\
% }
% It raises the demands to compute the $|J_1\cup\cdots\cup J_n|$.
% \paragraph{Theorem 1}
% $P(J_i) = \frac{\sum_{k=1}^n\frac{1}{k}A_i^k}{|J_1\cup\cdots\cup J_n|}$ is a probability distribution, where $A_{i}^k$ is the number of the tuples of $k$-th overlapped. %(TODO: Needs to calculate $A_i^k$)


% \begin{proof}
% We are going to show that $\sum_{i} P(J_i) =1 $. 
% \begin{align*}
%     \sum_{i=1}^{n} P(J_i) &=\sum_{i=1}^{n}\frac{\sum_{k=1}^n\frac{1}{k}A_i^k}{|J_1\cup\cdots\cup J_n|}\\
%     & =\frac{\sum_{k=1}^n \sum_{i=1}^{n} \frac{1}{k}A_i^k}{|J_1\cup\cdots\cup J_n|}\\
%     & = \frac{|J_1\cup\cdots\cup J_n|}{|J_1\cup\cdots\cup J_n|}=1
% \end{align*}
% \end{proof}

% The pair-wise overlapping information is not sufficient to compute $|J_1\cup\cdots\cup J_n|$.

% We would like to investigate the bound we have, there are two possible approaches, the first is to evaluate the $\frac{1}{2}\sum_{ki} O_{ik} - \sum_{k=2}^n\frac{1}{k}A_i^k $, and the alternative one is to evaluate the $ \frac{|J_i| \cdot ( 2\sum_i A_i^1 +\sum_{i} \sum_{k} O_{ik})}{C \cdot (\sum_{k} O_{ik}+2A_i^1)}$.

% Since original acceptance rate $= \frac{|J_i| }{\frac{1}{2}\sum_{k \neq i} O_{ik} }$, we need to bound $|J_i|$ below and bound $O_{ik}$ above.

% \subsection{Estimating $|J_i|$}
% Given $J_1 = R_1 \bowtie R_2 \bowtie R_3$, assuming 1-1 join, we have
% $$? \leq |J_1| \leq \min\{|R_1 \bowtie R_2|, |R_2 \bowtie R_3|, |R_1 \bowtie R_3|\}$$
% Assume key same attribute 
% $$|J_1| \geq |R_1 \cap R_2 \cap R_3|$$


% The following theorem is based on Containment assumption: when joining two tables, the set of values in the join column with the smaller column cardinality is a subset of the set of values in the join column with the larger column cardinality.
% \paragraph{Theorem 2} Given join path $J_n = R_1 \bowtie \cdots \bowtie R_n$, where the column cardinality of primary keys of table $R_i$ is $d_i, i = 1,2,\dots,n$, we have \cite{1994_join_size}
% $$|J_n| = d \times \frac{|R_1|}{d_1} \times \frac{|R_2|}{d_2} \times \cdots \frac{|R_n|}{d_n}, \text{ where } d = \min\{d_1,d_2,\dots,d_n\}$$

% \begin{proof}
% We first consider the case $J_1 = R_1 \bowtie R_2$ and assume uniformity of attribute values, i.e. the distinct values in a join column appear equi-frequently in the column. Thus we can obtain that number of tuples that contain a distinct value in $R_i$ is $\frac{|R_i|}{d_i}$. Then note that the number of distinct values appear in the join columns of $R_1 \bowtie R_2$ should be $\min\{d_1,d_2\}$, \textcolor{blue}{using the containment assumption}, we obtain
% $$|J_1| = |R_1 \bowtie R_2| = \min\{d_1,d_2\} \times \frac{|R_1|}{d_1} \times \frac{|R_2|}{d_2} = |R_1| \times |R_2| \times \frac{1}{\max\{d_1,d_2\}}$$
% since $\min\{d_1,d_2\}/(d_1\times d_2) = 1/\max\{d_1,d_2\}$.\\
% \textcolor{blue}{
% TODO:\\
% prove for general case (mathematical induction)\\
% release uniformity assumption\cite{1981_join_size}\\
% release containment assumption (change to intersection information)\\
% Let $d_{1,2}$ denote the column cardinality of primary key of $|R_1 \cap R_2|$, then
% $$|J_1| = |R_1 \bowtie R_2| = (d_1+d_2-d_{1,2}) \times \frac{|R_1|}{d_1} \times \frac{|R_2|}{d_2}$$
% }
% \end{proof}

% \subsection{Estimating $O_{12} = |J_1 \cap J_2|$}
% We need to bound $O_{12}$ above.
% \paragraph{Theorem 2} Let $\mathcal{C}_{i,k}$ be the join attribute of $R_i$ and $R_k$.
% Define $$R_i^k = \pi_{\mathcal{C}_{i,k}}(R_i)$$
% $$R_k^i = \pi_{\mathcal{C}_{i,k}}(R_k)$$
% \textcolor{blue}{We need to redefine what we need here.\\}
% \textcolor{blue}{Specify the $\mathcal{C}_{i,k}$ here.\\}
% Then we define $$N_i^k = N_k^i = \max\{|R_i^k \cap R_k^i|, 1\}$$
% \textcolor{blue}{$N_i^k$ tells us how much they overlap on the join attributes.\\}
% Now given $J_1 = R_{1,1} \bowtie \cdots \bowtie R_{1,n}, J_2 = R_{2,1} \bowtie \cdots \bowtie R_{2,m}$, we have
% $$|J_1 \cap J_2| \leq \prod_{i=1}^n\left(\prod_{k=1}^m N_{1,i}^{2,k}\right)$$
% \begin{proof}
% Let $J_1 \cap J_2$ = $R$ We prove by mathematical induction.\\
% The base case can be separated into the following 2 cases:
% \begin{enumerate}
%     \item $J_1 = R_{1,1}(A,B,C), \;J_2 = R_{2,1}(A,B) \bowtie R_{2,2}(B,C)$\\
%     Since two tables can be joined together only if they have same values on the join attributes, and $N_{1,1}^{2,1} \cdot N_{1,1}^{2,2}$ has counted all combinations, it's trivial that $$|J_1 \cap J_2| \leq N_{1,1}^{2,1} \cdot N_{1,1}^{2,2}$$
%     \textcolor{blue}{$J_1 = R_{1,1}(A,B,C), \;J_2 = R_{2,1}(A,B) \bowtie R_{2,2}(B,D)$\\}
%     \item $J_1 = R_{1,1}(A,B) \bowtie R_{1,2}(B,C), \;J_2 = R_{2,1}(A,B) \bowtie R_{2,2}(B,C)$\\
%     Suppose $t \in J_1 \cap J_2$, then $t\in J_1$ and $t\in J_2$, which gives us $\pi_{(A,B)}(t) \in R_{1,1}$ and $\pi_{(A,B)}(t) \in R_{2,1}$. Hence $$\pi_{(A,B)}(t) \in R_{1,1} \cap R_{2,1}$$
%     (Then if we show that $d_{A,B}(\pi_{(A,B)}(t),R)= |R_{1,1} \cap R_{2,1}|$)\\
%     Thus 
%     $$|J_1 \cap J_2| \leq N_{1,1}^{2,1} \cdot N_{1,1}^{2,2} \cdot N_{1,2}^{2,1} \cdot N_{1,2}^{2,2}$$
% \end{enumerate}
% \end{proof}

% Given $J_1 = R_1, J_2 = R_2 \bowtie R_3$\\

% \noindent Given $J_1 = R_1 \bowtie R_2, J_2 = R_2 \bowtie R_3 \bowtie R_4$, we claim
% $$O_{12} = |J_1\cap J_2| \leq |R_1 \cap R_3|$$
% Given $J_1 = R_{11} \bowtie R_{12} \bowtie R_{13}, J_2 = R_{21} \bowtie R_{22} \bowtie R_{23} \bowtie R_{24}$, we claim
% \begin{align*}
%     O_{12} &= |J_1\cap J_2|\\
%     &= |(R_{11} \bowtie R_{12} \bowtie R_{13}) \cap (R_{21} \bowtie R_{22} \bowtie R_{23})|\\
%     &\leq \min\{|(R_{1i} \bowtie R_{1j}) \cap (R_{2l} \bowtie R_{2m})|, i,k = 1,2,3,\;l,m=1,2,3,4\}
% \end{align*}\\
% Given $J_1 = R_{11} \bowtie \cdots \bowtie R_{1n}, J_2 = R_{21} \bowtie \cdots \bowtie R_{2m}$, we claim
% \begin{align*}
%     O_{12} &= |J_1\cap J_2|\\
%     &\leq \min\{|(R_{1i} \bowtie R_{1j}) \cap (R_{2k} \bowtie R_{2l})|, i,j = 1,\dots,n,\;k,l=1,\dots,m\}
% \end{align*}
% \begin{itemize}
%     \item Scenarios
%     \item Different keys, join paths(chain, star, cyclic)
%     \item Consider all as DAG
% \end{itemize}

% \subsection{Estimate $A_i^1$}
% For a loose upper bound, we claim
% $$A_i^1 = |J_i| - \max_{j}O_{ij}$$
% However, it is a really bad lower bound. We might want to have a better estimation.
% Based on $\sum_{k=1}^nA_i^k=|J_i|$, $A_i^1=|J_i|-\sum_{k=2}^n A_i^k$. For the possible theoretical analysis, we need to evaluate the $A$ and $O$.
% For an example in the Figure 1, it's simple. $A_i^2=\sum_{j}|O_{ij}|-\frac{1}{2}|O_{ijk}|$. We need to have a generalised one.

% \subsection{How to choose $C$}

\section{Sampling Disjoint Union}
\label{sec:disjointunion}

We first solve the disjoint union case which is simpler. Given the disjoint union $V = \{J_1\sqcup\ldots\sqcup J_n\}$,  we first select a join path $J_j$ with probability $P(J_j) = \frac{|J_j|}{|J_1+\ldots+J_n|}$. 
\fn{After selecting a join path $J_j$, we  select a random tuple from $J_j$. We repeat the process until $N$ sampled tuples are obtained.}

\begin{algorithm}
\caption{Disjoint Union of Joins Sampling}
\begin{small}
\begin{algorithmic}[1]
\Require{Join paths $S = \{J_j, 1\ \leq j \leq n\}$, Tuple count $N$}
\Ensure{Sample $T = \{t_i, 1 \leq i \leq N\}$}
\State $\fn{T} \leftarrow \{\}$ \Comment{target sample}
% fn: let's remove the warmup phase from the pseudo code
%\For{i = 1,2,\dots, n}
%\State Estimate $|J_i|$ 
%\EndFor
\While{$n < N$}
\State $J \leftarrow$ a random join path $J_j$ with probability $\frac{|J_j|}{\sum_{j=1}^n |J_j|}$
\State $t \leftarrow$ a sample from $J$ using hashing approach of \S~\ref{sec:samplejoin}
\State add $t$ to $T$
\State $n \leftarrow n + 1$
\EndWhile
\State \textbf{return} $T$
\end{algorithmic}
\label{alg1}
\end{small}
\end{algorithm}

Algorithm~\ref{alg1} shows the pseudocode for sampling a disjoint union. In Line 4, the algorithm needs to take a random sample from a join paths. Methods of sampling a tuple from a single join path has long been a popular problem~\cite{?}. 
%, and multiple efficient ways for different types of join paths are proposed in recent years. %We leave a 
\fn{In \S~\ref{sec:samplejoin}, we propose an efficient way of sampling from a join path by relying on  limited data statistics.} \fn{FN: briefly mention how it is different than existing work.}

\begin{theorem}
Given \fn{join paths $S=\{J_1,\ldots, J_n\}$, Algorithm~\ref{alg1} return each result tuple $t$ with probability $\frac{1}{|J_1+\ldots+J_n|}$.} 
%the probability of selecting a tuple $t$ from the disjoint union of join paths,} $V = \{J_1\sqcup\ldots\sqcup J_n\}$, 
%disjoint union of  $J_j's$, 
%the probability of selecting a tuple $t_0$ from $V$ is $\frac{1}{|J_1+\ldots+J_n|}$. 
\end{theorem}
\begin{proof}
\begin{align*}
     P(t) = \frac{|J_j|}{|V|} \cdot \frac{1}{|J_j|} = \frac{1}{|V|}
\end{align*}
\end{proof}

In order to calculate the probability distribution of join paths, we need to estimate $|J_j|$ for all $j$ before the sampling process. There are various of ways of estimating a join size which we revisit  next. 
Regardless of the choice of join estimation, Algorithm~\ref{alg1} always returns independent samples since returned sample is always uniform regardless of the history of samples, \fn{as long as we guarantee a  result tuple from a selected $J_j$ is sampled with the estimated  probability $1/|J_j|$.} 

\subsection{Join Size Estimation Revisited}
\label{sec:joinsize}

\fn{There is a consistent interest in the database theory community in upper bounding a join size~\cite{citeallworks}.  
Our sampling framework allows us to plug in any of these estimations. Olken proposed a way of estimating the size of join paths of two relations~\cite{Olken}. Here, we extend Olken's algorithm to calculate the upper bound on the size of join paths of  arbitrary number of relations. } \fn{Assume a join path $J = R_1 \bowtie_{A_1} R_{2} \bowtie_{A_2} \cdots \bowtie_{A_{n-1}} R_{n}$. Let $M_{A_i}(R_{i+1})$ be the maximum value frequency in  attribute $A_i$ of relation  $R_{i+1}$. We have the following upper bound for the size of a join path $J$.
$$|J| \leq |R_{1}| \cdot \prod_{i = 1}^{n-1} M_{A_i}(R_{i+1})$$}

\textcolor{blue}{Could later add AGM bound\cite{agm}}


\section{Sampling Set Union}
\label{sec:setunion}

\fn{Given the set union $U = \bigcup_{j = 1}^n J_j$,  we first select a join path $J_j$ with some probability distribution then select a random tuple from $J_j$. This process is repeated until $N$ unique sampled tuples are obtained.} We assume that there is no duplicates in each join path $J_j$. To guarantee that for each sampled tuple $t$, $P(t)=\frac{1}{\vert U \vert}$, we need to take the tuples that lie in overlapping areas into consideration. We first separate each join path $J_j$ into $n$ \fn{disjoint} parts, denoted as $J_j = \bigcup_{k = 1}^n \mathcal{A}_j^k$, where $\mathcal{A}_{j}^k$ is the set  of tuples of $k$-th overlapped in $J_j$. That is, each tuple in $\mathcal{A}_j^k$ \fn{belongs to $J_j$ and appears in exactly $k-1$ other join paths.}  
%also appears in other $k-1$ join paths except $J_j$. 
\begin{example}
Figure~\ref{fig:ajk} represents the $\mathcal{A}_{j}^k$ areas for relation $J_1$, where the red area is $\mathcal{A}_{j}^1$, the blue area is $\mathcal{A}_{j}^2$, and the green area is $\mathcal{A}_{j}^3$. 
\end{example}

Since for each $J_j$,  $\mathcal{A}_{j}^k$'s are disjoint, \fn{we can define the set union $U$ as follows.}
\begin{equation}
\label{eq:Ajk}
|U| = \sum_{j=1}^n\sum_{k=1}^n\frac{1}{k}\mathcal{A}_j^k
\end{equation}

\eat{
\begin{example} 
Figure~\ref{fig:ajk} represents $\mathcal{A}_{j}^k$ areas, where the red area is $\mathcal{A}_{j}^1$, the blue area is $\mathcal{A}_{j}^2$, and gthe reen area is $\mathcal{A}_{j}^3$. 
Considering the data of Table~\ref{tab:joinpathexample} for these join paths, we then have $\mathcal{A}_1^2 = \mathcal{A}_2^2 = (3,6,4)$.
The set of remaining elements in $J_1$ is $A_1^1$, and similarly the set of remaining elements in $J_2$ is $\mathcal{A}_2^1$.
\end{example}}

Note that $\mathcal{A}_j^k$ is a non-trivial information, \fn{since evaluating the overlap of two or more join paths requires performing join and computing $k$-way overlaps of join results. We will provide a solution for approximating $\mathcal{A}_j^k$'s in \S~\ref{sec:koverlap}}. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/overlap.png}
    \vspace{-5mm}
    \caption{$\mathcal{A}_j^k$ areas for three join paths. \fn{FN: how about integrating tuples of table 1 in this figure?}}
    \label{fig:ajk}
\end{figure}

\fn{Algorithm~\ref{alg2} shows the pseudocode for sampling from a set union of join paths. The algorithm selects a join path $J_j$ with probability \eat{$P(J_j) = \frac{|J_j|}{|U|}$}\yurong{$P(J_j) = \frac{|J_j|}{\sum_{j\in[n]}|J_j|}$}, then selects a random tuple $t$ from $J_j$. By definition, tuple $t$ lies exactly in one area of $J_j$, say $\mathcal{A}_j^k$. When $k=1$, tuple $t$ does not exist in any other join paths. 
When $k>1$, tuple $t$ appears in exactly $k$ join paths and has $k$ times  probability to be selected from the disjoint union compared to tuples in $\mathcal{A}_j^1$. 
\yurong{Note set union disregards duplicates.} Therefore, $t$ is rejected with some probability, such that the probability of $t$ becomes $1/|U|$.
% Hence, we first define a rejection rate $1-\frac{1}{k}$ for $t$.} 
} 
\eat{
Given information of $\mathcal{A}_j^k$, we define a rejection rate to ensure uniformity when sampling a tuple. 
Suppose the probability of selecting a join path is $P(J_j)$, then the probability of tuple $t_v$ with value $v$ randomly selected from $J_j$ is $\frac{1}{|J_j|} * P(J_j)$, which lies exactly in one area of $J_j$, say $\mathcal{A}_j^{k_0}$. 
We define $P(J_j) = \frac{|J_j|}{|U|}$ to make sure every tuple in every join path has the same probability $\frac{1}{|U|}$ to be selected.
When $k_0 = 1$, there are no other tuples with value $v$ in any other joins, then $P(t_v) = \frac{1}{|U|}$. When $k_0 > 1$, we still want $P(t_v) = \frac{1}{|U|}$. But given that there a total number of $k_0$ tuples with value $v$ in all the join paths, it has $k_0$ times  probability to be selected compared to tuples in $\mathcal{A}_j^1$. Hence we reject $t_v$ in $\mathcal{A}_j^{k_0}$ with probability $1-\frac{1}{k}$.} 
Nevertheless, identifying which area $t$ comes from is expensive as we should \fn{execute all join paths and access their data}.  
%the underlying data. 
Therefore, the algorithm defines a probability distribution to predict the area to which the  selected $t$ belongs. Let $P(\mathcal{A}_j^k | t\in J_j)$ denote the probability of $t$ coming from $\mathcal{A}_j^k$. 
\begin{equation}
\label{eq:pAjkt}
P(\mathcal{A}_j^k | t\in J_j) = \frac{|\mathcal{A}_j^k|}{|J_j|}
\end{equation}
\fn{Depending on the selected $k$, the acceptance rate of tuple $t$ is $\frac{\sum_{j\in[n]}{|J_j|}}{k\cdot|U|}$.} 
\yurong{Then since our goal is to ensure that each tuple $t$ from the set union has probability $\frac{1}{|U|}$ to be selected, we define another acceptance rate $\frac{|J_j|\cdot \sum_{j\in[n]}|J_j|}{|U|^2}$ for all the tuples in all join paths.
Therefore, combined with the previous rejection rate, we have Algorithm~\ref{alg2} rejects $t$ from $\mathcal{A}_j^k$ with probability $1-\frac{|J_j|\cdot\sum_{j\in[n]}|J_j|}{k\cdot |U|^2}$.}

\yurong{However, note that $\frac{|J_j|\cdot\sum_{j\in[n]}|J_j|}{k\cdot |U|^2}$ can be greater than 1. In this case, we utilize a trick to modify the probability. Suppose $t$ has acceptance rate $p > 1$, then we accept $\lfloor p \rfloor$ number of $t$ with probability $1$, and another $t$ with probability $p-\lfloor p \rfloor$. In this way, we can guarantee that the expected number of $t$ we get is
\begin{equation}
    E(t) = \lfloor p \rfloor \cdot 1 + 1 \cdot (p-\lfloor p \rfloor) = p
\end{equation}}

\eat{
\paragraph{Lemma} Given set union $U = J_1 \bowtie J_2 \bowtie \cdots \bowtie J_n$, we have
\begin{align*}
    |U| &= |J_1 \bowtie J_2 \bowtie \cdots \bowtie J_n|\\
    &= \sum_{j=1}^n\sum_{k=1}^n\frac{1}{k}\mathcal{A}_j^k
\end{align*}
\begin{proof}
\textcolor{blue}{I temporarily leave the proof blank. Not sure what level of proof we need to provide for this lemma as it's pretty intuitive}
\end{proof}
}

\begin{theorem}
\label{th:setunioniid} 
\fn{Given join paths $S=\{J_1,\ldots, J_n\}$, the \textcolor{cyan}{expected} probability of returning  %selecting \yurong{and accepting} 
a tuple $t$ from the set union of join paths 
$U = \{J_1\cup\ldots\cup J_n\}$, using Algorithm~\ref{alg2} 
is $\frac{1}{|J_1\cup\ldots\cup J_n|}$.} 
%For each $t_i$ in join path $J_j$, the expected probability of selecting $t_i$ is $P(t_i) = \frac{1}{\vert U \vert}$.
\end{theorem}
\begin{proof}
\fn{A join path $J_j$ is selected with probability  $|J_j|/\sum_{j\in[n]}|J_j|$ and  the probability of selecting $t$ from $J_j$ is 
$1/|J_j|$.  } 
%\textcolor{red}{The problem here is that $|J_j|/|U|$ is not a distribution, we have to use $|J_j|/\sum |J_j|$. However, it raises the problem that at the end we need multiply $\sum |J_j|/|U|$ to achieve the goal. } 
\fn{Tuple $t$ belongs to area   $\mathcal{A}_j^k$ with probability  $|\mathcal{A}_j^k|/|J_j|$ and is accepted with probability $\frac{\sum_{j\in[n]}{|J_j|}}{k\cdot|U|}$.
\eat{Therefore, the probability of selecting $t$ from $J_j$ is as follows. 
\begin{align*}
P(t\in J_j) &=  \frac{|J_j|}{\sum_{j\in[n]}|J_j|} \cdot \frac{1}{|J_j|} \cdot \sum_{k=1}^n \frac{\sum_{j\in[n]}{|J_j|}}{k\cdot|U|} \cdot P(\mathcal{A}_j^k | t)\\
&= \frac{1}{|U|}\sum_{k=1}^n \frac{1}{k}\cdot P(\mathcal{A}_j^k | t)
\end{align*}
We know tuple $t$ can be selected from any join paths. Therefore, from Equation~\ref{eq:pAjkt}, the expected probability of selecting $t$
 from $U$ is as follows.} }
\eat{
\begin{align*}
    P(t) &= \sum_{j=1}^n \left( \frac{|J_j|}{|U|} \cdot \frac{1}{|J_j|} \cdot \sum_{k=1}^n \frac{1}{k} |\mathcal{A}_j^k|\right)/ |U|\\
    &= \left(\frac{1}{|U|} \cdot \sum_{j=1}^n \sum_{k=1}^n \frac{1}{k} |\mathcal{A}_j^k|\right) / |U|\\
    &= \left(\frac{1}{|U|} \cdot |U|\right) /|U|\\
    &= \frac{1}{|U|}
\end{align*}
\begin{align*}
    P(t) &= \sum_{j=1}^n \left( \frac{1}{|U|} \cdot \sum_{k=1}^n \frac{1}{k} |\mathcal{A}_j^k|\right)/ |U|\\
    &= \left(\frac{1}{|U|} \cdot \sum_{j=1}^n \sum_{k=1}^n \frac{1}{k} |\mathcal{A}_j^k|\right) / |U|\\
    &= \left(\frac{1}{|U|} \cdot |U|\right) /|U|\\
    &= \frac{1}{|U|}
\end{align*}
}


\yurong{Therefore, from Equation~\ref{eq:pAjkt}, the expected probability of selecting $t$ from $U$ is as follows.
\begin{align*}
P(t) &= P(J_j) \cdot P(t \text{ accepted } \vert J_j)\\
&= \sum_{j=1}^n \left( \frac{|J_j|}{\sum_{j\in[n]}|J_j|} \cdot \frac{1}{|J_j|} \cdot \sum_{k=1}^n \frac{|A_j^k|}{|J_j|}\cdot \frac{|J_j|\cdot\sum_{j\in[n]}|J_j|}{k\cdot |U|^2} \right) \\
&= \frac{1}{|U|^2} \cdot \left(\sum_{j=1}^n \sum_{k=1}^n \frac{1}{k} |\mathcal{A}_j^k|\right)\\
&= \frac{1}{|U|^2} \cdot |U|\\
&= \frac{1}{|U|}
\end{align*}
since from Equation~\ref{eq:Ajk}, we have $|U| = \sum_{j=1}^n \sum_{k=1}^n \frac{1}{k} |\mathcal{A}_j^k|$.}
\end{proof}

% \textcolor{cyan}{Then we prove that the expected probability of selecting any $t$ from $U$ is $\frac{1}{|U|}$. Equivalently, we show $\sum_{t \in U}P(t \text{ accepted}) = 1$.
% Consider the discrete space $U$, which is the set of the join tuples under the set union operations. Then $\forall u \in U$, we want to make sure that $P(t=u) = \frac{1}{|U|}$. 
% \begin{align*}
% P(t=u) &= \left(\sum_{t \in U}P(t \text{ accepted})\right) / |U|\\
% &= \sum_{j=1}^n \left( \frac{|J_j|}{\sum_{j\in[n]}|J_j|} \cdot \frac{1}{|J_j|} \cdot \sum_{k=1}^n |A_j^k|\cdot \frac{\sum_{j\in[n]}|J_j|}{k\cdot |U|} \right)/|U| \\
% &= \left(\sum_{j=1}^n \sum_{k=1}^n \frac{1}{k} |\mathcal{A}_j^k| \cdot \frac{1}{|U|}\right)/|U|\\
% &= \left(|U| \cdot \frac{1}{|U|}\right)/|U|\\
% &= \frac{1}{|U|}
% \end{align*}}
% Aug 12
\textcolor{violet}{
\subsection{Bernoulli Case}
We first define a Bernoulli distribution over each join path with $P(J_j \text{ is chosen}) = \frac{|J_j|}{|U|}$. Algorithm \ref{algU} shows the process of calculating $|U|$, and we'll further introduce the algorithm for $O$'s and $\mathcal{A}$'s in the following sections. Consider the discrete space $U$, which is the set of the join tuples under the set union operations. Then $\forall u \in U$, we want to make sure that $P(t=u) = \frac{1}{|U|}.$ Algorithm \ref{algB} then shows the pseudocode for sampling from a set union of join paths using a Bernoulli distribution. The algorithm iterates through all the join paths every round, and each join path is selected \yurong{(yl: not sure which word to use here; could change to other words like accept/chosen)} with probability $\frac{|J_j|}{|U|}$. We use $P(J_j)$ to denote the probability of $J_j$ being selected. If join path $J_j$ is selected, we randomly sample a tuple $t$ from it. Let $t.v$ denote the value of tuple $t$, and $J(t.v)$ denote the join path the first time $t.v$ is sampled from. Suppose it's the first time a tuple with value $u$ is sampled, then we assign $J(u) = J_j$, and accept the tuple; if it's not, then we accept the tuple if $J(u) = J_j$, and reject it otherwise. We now prove that this algorithm returns every $u \in U$ with probability $\frac{1}{|U|}$.
\begin{theorem}
Given join paths $S=\{J_1,\ldots, J_n\}$, the  probability of returning a tuple $t$ with value $u$ from the set union of join paths $U = \{J_1\cup\ldots\cup J_n\}$, using Algorithm~\ref{algB} 
is $\frac{1}{|J_1\cup\ldots\cup J_n|}$.
\end{theorem}
\begin{proof}
Let $J(u)$ be the the join path the first time tuple with value $u$ is selected from. Let $\Delta(u)$ be the set of join paths that contain tuple with value $u$. Then we have
\begin{align*}
    P(t = u) &= \sum_{J_j \in S} P(J_j) \cdot P(t = u \vert J_j)\\
    &= \frac{|J(u)|}{|U|} \cdot \frac{1}{|J(u)} + \sum_{J_j \in \Delta(u)\backslash J(u)} \frac{|J_j|}{|U|} \cdot \frac{1}{|J_j|} \cdot 0 + \sum_{J_j \in S\backslash \Delta(u)} 0\\
    &= \frac{1}{|U|} + 0 + 0\\
    &= \frac{1}{|U|}
\end{align*}
\end{proof}}

\begin{algorithm}
\caption{Estimating $|U|$}
\begin{small}
\begin{algorithmic}[1]
\Require{Join paths $S = \{J_j, 1\ \leq j \leq n\}$, Tuple count $N$}
\Ensure{$|U|$}
\For{j = 1,2,\dots, n}
\State Estimate $|J_j|$ 
\EndFor
\For{k = n,n-1,\dots, 1}
\For{each power set $\Delta_k$ of $S$}
\State Estimate $|\mathcal{O}^k_{\Delta_k}|$ 
\EndFor
\For{j = 1,2,\dots, n}
\State Calculate $|\mathcal{A}_j^k|$
\EndFor
\EndFor
\State \textbf{return} $|U| = \sum_{j=1}^n\sum_{k=1}^n\frac{1}{k}\mathcal{A}_j^k$
\end{algorithmic}
\label{algU}
\end{small}
\end{algorithm}

\begin{algorithm}
\caption{Set Union of Bernoulli Joins Sampling}
\begin{small}
\begin{algorithmic}[1]
\Require{Join paths $S = \{J_j, 1\ \leq j \leq n\}$, Tuple count $N$, Set union size $|U|$}
\Ensure{Tuples $\{t_i, 1 \leq i \leq N\}$}
\State $S \leftarrow \{\}$ \Comment{target sample}
\While{$n < N$}
\For{$j = 1$ to $n$}
\State choose $J_j$ with probability $\frac{|J_j|}{|U|}$
\If{$J_j$ is chosen}
\While{$t \in round\_record$}
\State $t \leftarrow$ a random sample from $J_j$
\EndWhile
\If{$t \in S$}
\If{$J(t(u)) == J_j$}
\State accept $t$ with probability 1
\Else
\State reject $t$ with probability 1
\EndIf
\Else 
\State accept $t$ with probability 1
\EndIf
\If{$t$ is accepted}
\State add $t$ to $S$; $J(t.u) = J_j$
\State add $t$ in $round\_record$
\State $n \leftarrow n + 1$
\EndIf
\EndIf
\EndFor
\EndWhile
\State \textbf{return} $S$
\end{algorithmic}
\label{algB}
\end{small}
\end{algorithm}

\textcolor{violet}{
\subsection{Non-Bernoulli Case}
We now propose our second solution for the set-union case.}
\begin{algorithm}
\caption{Set Union of Non-Bernoulli Joins Sampling}
\begin{small}
\begin{algorithmic}[1]
\Require{Join paths $S = \{J_j, 1\ \leq j \leq n\}$, Tuple count $N$, Set union size $|U|$}
\Ensure{Tuples $\{t_i, 1 \leq i \leq N\}$}
\State $S \leftarrow \{\}$ \Comment{target sample}
\While{$n < N$}
\State $J \leftarrow$ a random join path $J_j$ with probability $\frac{|J_j|}{|\sum_{j\in[n]}|J_j|}$
\State $t \leftarrow$ a sample from $J$ 
\If{$t \in S$}
\If{$t(u).J == J$}
\State accept $t$ with probability $\frac{|\sum_{j\in[n]}|J_j|}{|U|}$
\Else
\State reject $t$ with probability 1
\EndIf
\Else 
\State accept $t$ with probability $\frac{|\sum_{j\in[n]}|J_j|}{|U|}$
\EndIf
\If{$t$ is accepted}
\State add $t$ to $S$; $t(u).J = J$
\State $n \leftarrow n + 1$
\EndIf
\EndWhile
\State \textbf{return} $S$
\end{algorithmic}
\label{algNB}
\end{small}
\end{algorithm}

\eat{
\begin{algorithm}
\caption{Set Union of Joins Sampling}
\begin{small}
\begin{algorithmic}[1]
\Require{Join paths $S = \{J_j, 1\ \leq j \leq n\}$, Tuple count $N$}
\Ensure{Tuples $\{t_i, 1 \leq i \leq N\}$}
\State $S \leftarrow \{\}$ \Comment{target sample}
\For{j = 1,2,\dots, n}
\State Estimate $|J_j|$ 
\EndFor
\For{k = n,n-1,\dots, 1}
\For{each power set $\Delta_k$ of $S$}
\State Estimate $|\mathcal{O}^k_{\Delta_k}|$ 
\EndFor
\For{j = 1,2,\dots, n}
\State Calculate $|\mathcal{A}_j^k|$
\EndFor
\EndFor
\While{$n < N$}
\State $J \leftarrow$ a random join path $J_j$ with probability
% $\frac{\sum_{k=1}^n\frac{1}{k}A_j^k}{|J_1\cup\cdots\cup J_n|}$ or
\yurong{$\frac{|J_j|}{|\sum_{j\in[n]}|J_j|}$}
\State $k \leftarrow$ a random number from $1$ to $n$ chosen with probability $|\mathcal{A}_j^k| / |J_j|$
\State \yurong{accept with probability $\frac{\sum_{j\in[n]}{|J_j|}}{k\cdot|U|}$}
\If{not rejected}
%\If{$t$ is not rejected}
\State \fn{$t \leftarrow$ a sample from $J$ using hashing approach}
\State add $t$ to $S$
\State $n \leftarrow n + 1$
\EndIfop
\EndWhile
\State \textbf{return} 
\end{algorithmic}
\label{alg2}
\end{small}
\end{algorithm}
}

\eat{Following the framework we discussed above, Algorithm~\ref{alg2} shows the pseudocode for the set union case. After selecting a tuple $t$ from the selected join path, we randomly generate a number $k$ in range $1$ to $n$ to predict which overlapping area $t$ comes from, and reject it with probability $1-\frac{1}{k}$. }
\fn{In Algorithm~\ref{alg2}, during the warm-up phase before the sampling process, we need to estimate the join size for all join paths $J_j$  as described in \S~\ref{sec:joinsize}. 
%What's more, 
The naive solution to calculate the ratio of} each overlapping area in each join path ($\mathcal{A}_j^k$'s) would be to generate and iterate through all power sets of $S = \{J_1,\dots,J_n\}$, then  \fn{execute the joins and overlaps}. \fn{FN: is there any way besides brute force and approximation?} 

\fn{Next, we propose} 
ways of estimating $\mathcal{A}_j^k$ \fn{using  the pairwise overlap of join paths which is much cheaper to compute. Then, we describe how to estimate pairwise overlaps  using XX. } \yurong{yl: we are using general overlap to estimate $\mathcal{A}$}

\fn{First, we define $k$-way overlaps. Let $c\subseteq S$ be a set of join paths and $O_c$ be the set of tuples in the intersection of join paths in $c$. Let $\Delta_k$ be a  $k$-combination of join paths in $S$, i.e., the a subset in the powerset of size $k$ of $S$.   We use $\mathcal{O}_{\Delta_k}$ to denote the overlapping tuples of join paths  $\Delta_k$ %such that join path $J_j\in c$, 
i.e., $\mathcal{O}_{\Delta_k} = \cap_{J_j\in\Delta_k} J_j$.} 
\fn{Note that $\mathcal{O}_{j}^k$ is the set of tuples of $J_j$ that appear in any $k-1$ other join paths in $S$, while $\mathcal{A}_j^k$ is the set of tuples of $J_j$ that appear in {\em exactly} $k-1$ other join paths. } 
\fn{FN: please double check this.}
\subsubsection{Controlling the final steps}
\draco{The last few steps might be out of control. The inflation rate is for sure larger or equal than 1, thus we could not control how many samples we generate in each step if the inflation rate doesn't happen to be int. Here we formalize it to a mathmatical expression.}
\draco{Let $R$ be the inflation rate, which is $\frac{\sum_{i}J_i}{|U|}$, we define the $r_i$ be the prob that $i$ sample be generated in a certain round. Then we have:  }

\begin{align*}
   \sum_{i}^n r_i \cdot i =R\\
   \sum_{i}^n r_i = 1 \\
   0\leq r_i \leq 1
\end{align*}
, where $n \in N^+ $. When $n>R$, this system has infinitely many solutions. Any valid solution could be taken for controlling the number of samples in the last round. For example, by the last round we are missing $j$ samples. We pick a solution of the system such that $r_j \neq 0$, then for sure we could obtain exactly $j$ samples from the last iteration by discarding if we fall into $r_i$ cases when $i \neq j$.


\section{Join Path Overlap}
\label{sec:joinoverlap} 

\fn{In order to estimate the $k$-overlaps, $\mathcal{A}_j^k$'s, we first introduce a way of estimating the overlap of two join paths of the same length (number of relations). Then, we describe a way of bounding the overlap of more than two such join paths. Building on this bound, we  relax the assumption on the length of join paths and solve the problem for the generic case of join path overlap, $\mathcal{O}_{\Delta}$. Finally, we propose a way of estimating $\mathcal{A}_j^k$'s from join path  overlaps.} 

\subsection{Overlap of Two Join Paths}

\fn{Given two join paths $J = R_{1} \bowtie_{A_{1}} R_{2} \bowtie_{A_{2}} \cdots \bowtie_{A_{n_1-1}} R_{n_1}$, with  $n_1$ tables, and $J^\prime = R^\prime_{1} \bowtie_{A^\prime_{1}} R^\prime_{2} \bowtie_{A^\prime_{2}} \cdots \bowtie_{A^\prime_{n_2-1}} R^\prime_{n_2}$, with $n_2$ tables, we want to find an upper bound for the size of $|J \cap J^\prime|$.} 
\fn{Consider the simplest case where $J$ and $J^\prime$ are both chain joins of the same length, i.e., $n_1 = n_2$, and for each relation $R_i$ in $J$ there is a corresponding unionable relation $R^\prime_i$ in $J^\prime$. This allows us to order relations in join paths according to their unionability. %For example, $R_i$ of $J$ and $R^\prime_i$ of $J^\prime$ have schemas and attributes with one-to-one mappings. 
In other words, for now, we consider the special case where join paths are constructed from  relations with unionable schemas. We also assume that join attributes on the first two  relations of the join paths are unionable. For example, for the join $R_1 \bowtie_{A_{1}} R_2$ on relations $R_1$ and $R_2$ of $J$ and the join $R^\prime_1 \bowtie_{A^\prime_{1}} R^\prime_2$ on corresponding unionable relations $R^\prime_1$ and $R^\prime_2$ in $J^\prime$, we assume join attributes $A_1$ and $A^\prime_{1}$ are unionable.  We will relax these assumptions in \S~\ref{sec:overlapgeneral}.}  
Trivially, a loose upper bound for the \fn{overlap of} $J$ and $J^\prime$ is $\min\{|J|, |J^\prime|\}$.  
\fn{Let $J_1 = R_{1} \bowtie_{A_1} R_{2}$ and $J^\prime_1 = R^\prime_{1} \bowtie_{A^\prime_1} R^\prime_{2}$ denote the results of the first joins in $J$ and $J^\prime$. Since the joins can be many-to-many, we have $|J_1 \cap J^\prime_1| \leq |J \cap J^\prime| \leq \min\{|J|, |J^\prime|\}$. We define $\mathcal{K}(1) = \min\{|J_1|, |J^\prime_1|\}$.}  
Then, we look at $J_2$ and $J^\prime_2$ defined as  $J_2 = R_1 \bowtie_{A_1} R_2 \bowtie_{A_2} R_3 = J_1 \bowtie_{A_2} R_3$ and $J^\prime_2 = R^\prime_1 \bowtie_{A^\prime_1} R^\prime_2 \bowtie_{A^\prime_2} R^\prime_3 = J^\prime_1 \bowtie_{A^\prime_2} R^\prime_3$, respectively. Similarly, a loose upper bound for $|J_2 \cap J_2^\prime|$ is $\min\{|J_1  \bowtie_{A_2} R_3|, |J^\prime_1 \bowtie_{A^\prime_2} R^\prime_3|\}$.  Let $M_{A_l}(R_i)$ be  the maximum degree of values in relation $R_i$ on the join attribute $A_l$. We define $\mathcal{K}(2)$ as follows. 
\begin{align*}
    \mathcal{K}(2) &= \min\{|J_1 \bowtie_{A_2} R_3|, |J^\prime_1 \bowtie_{A^\prime_2} R^\prime_3|\}\\
    &\leq 
    %\min_{j,j^\prime}\{\mathcal{K}(1) \cdot M_{A_2}(R_{j,3})\}\\
    \min\{\mathcal{K}(1) \cdot M_{A_2}(R_3), \mathcal{K}(1) \cdot M_{A^\prime_2}(R^\prime_3)\}\\
    &= \mathcal{K}(1) \cdot \min\{ M_{A_2}(R_3), M_{A^\prime_2}(R^\prime_3)\}
\end{align*}
For the general case, we have 
\begin{align*}
     \mathcal{K}(i) &= \min\{|J_{i-1} \bowtie_{A_i} R_{i+1}|, |J^\prime_{i-1} \bowtie_{A^\prime_i} R^\prime_{i+1}|\}\\
     &\leq \min\{\mathcal{K}(i-1) \cdot M_{A_i}(R_{i+1}), \mathcal{K}(i-1) \cdot M_{A^\prime_i}(R^\prime_{i+1})\}\\
     &= \mathcal{K}(i-1) \cdot \min\{ M_{A_i}(R_{i+1}), M_{A^\prime_i}(R^\prime_{i+1})\}
\end{align*} 
\fn{This gives us $\mathcal{K}(n-1) = \min\{|R_1  \bowtie \cdots \bowtie R_n|, |R^\prime_1 \bowtie \cdots \bowtie R^\prime_n|\}$.
}
\fn{The overlap of two join paths with the same number of relations can be evaluated as follows.} 
\begin{align*}
    |J\cap J^\prime| &\leq \mathcal{K}(n-1)\\
    &= \mathcal{K}(n-2) \cdot \min\{ M_{A_{n-1}}(R_n), M_{A^\prime_{n-1}}(R^\prime_n)\}
\end{align*}
%Through this way, we can find the upper bound of pairwise join path overlapping size dynamically. 

This allows us to compute the pairwise join overlap recursively using the maximum degree of join attributes as well as the overlap between the join results of the first two relations in each join path. Next, we introduce two methods of estimating $\mathcal{K}(1)$. 

%\subsubsection{Extending Olken's algorithm}
% too short to be a subsection

One way is to follow Olken’s algorithm~\cite{Olken}. Let $\mathcal{N}(i)$ and $\mathcal{N}^\prime(i)$ be the upper bound of $|J_i|$ and $|J^\prime_i|$, respectively. For each tuple $t\in R_1$, a loose bound for the number of tuples in $R_2$ with which $t$ could join  is $M_{A_1}(R_2)$. Since there are $|R_1|$ tuples in $R_1$, we have
$\mathcal{N}(1) = |R_1| \cdot M_{A_1}(R_2)$. Similarly, we have $\mathcal{N}^\prime(1) = |R^\prime_1| \cdot M_{A^\prime_1}(R^\prime_2)$. Therefore, we get $\mathcal{K}(1) = \min\{\mathcal{N}(1), \mathcal{N}^\prime(1)\}$. 

%\subsubsection{Value based method} 

Note that Olken's method is tuple-based. Now, we propose our value-based approach. \fn{Let $\mathcal{D}_{A}(R)$ be the domain of values of attribute $A$ in relation $R$.} %Let $\mathcal{D}_{A_1} = \mathcal{D}_{A_1}(R_{1,1}) \cap \mathcal{D}_{A_1}(R_{1,2}) \cap \mathcal{D}_{A_1}(R_{2,1}) \cap \mathcal{D}_{A_1}(R_{2,2})$ be the overlap of all join attributes in relations of $J_{1,2}$ and $J_{2,2}$. }  
Let $d_{A_l}(v,R_i)$ denote the degree of value $v\in\mathcal{D}_{A_l}(R_i)$. Given $R_1 \bowtie_{A_1} R_2$, since we may have many-to-many joins, we have  the number of tuples with join attribute value $v$ obtained from the join to be $d_{A_1}(v,R_1) \cdot d_{A_1}(v,R_2)$.  Similarly, $d_{A^\prime_1}(v,R^\prime_1) \cdot d_{A^\prime_1}(v,R^\prime_2)$ bounds the number of tuples with join attribute value $v$ obtained from $R^\prime_1 \bowtie_{A^\prime_1} R^\prime_2$. 
Now we introduce an upper bound $\mathcal{K}(v,1)$ for the number of overlapping tuples with value $v$ after the first joins $J_1$ and $J_2$. For each Let $\mathcal{D}=\mathcal{D}_{A_1}(R_1)\cap\mathcal{D}_{A_1}(R_2)\cap\mathcal{D}_{A^\prime_1}(R^\prime_1)\cap\mathcal{D}_{A^\prime_1}(R^\prime_2)$. For each $v\in\mathcal{D}$, we have the following. $$\mathcal{K}(v,1) =
\min\{d_{A_1}(v,R_1) \cdot d_{A_1}(v,R_2), d_{A^\prime_1}(v,R^\prime_2) \cdot  d_{A^\prime_1}(v,R^\prime_2)\}$$
We can now aggregate over all values of $v$. 
$$\mathcal{K}(1) = \sum_{v \in \mathcal{D}} \mathcal{K}(v,1)$$

\fn{FN: would intersection of att domains work?}

\fn{how do we compute value-based K(1) in practice?}

% \subsection{Dynamic approach}
% We also propose a dynamic approach to estimate the overlapping size in an more accurate way. We employ the definition of $\mathcal{C}_{A_i}$ and $\mathcal{N}(v,i)$ from the value based method



% \subsection{Extending Chaudhuri et al.’s algorithm}


% Then for an upper bound of $O_{12}$, we have
% $$O_{12} \leq \sum_{v\in C_A} \mathcal{K}(v)$$
% Notice that $\argmax_{v\in C_A} K(v) = \argmax d_A(v,R_{j,1}) \cdot  d_A(v,R_{j,2})$ since $\min\{c_A(R_{j,3}),c_B(R_{j,3})\}$ stays the same for all $v$, so the equation can be reformulated as follows
% $$O_{12} \leq \min\{c_A(R_{j,3}),c_B(R_{j,3})\} \cdot \sum_{v\in C_A} \min_{j\in\{1,2\}}\{d_A(v,R_{j,1}) \cdot  d_A(v,R_{j,2})$$

% An example is as follows
% \begin{align*}
%     J_1 =& R_{1,1} \bowtie_A R_{1,2} \bowtie_B R_{1,3} \text{ where}\\
%     & d_A(v,R_{1,1}) = 10\\
%     & d_A(v,R_{1,2}) = 9\\
%     & c_B(R_{1,2}) = 7\\
%     & c_B(R_{1,2}) = 5\\
%     \\
%     J_2 =& R_{2,1} \bowtie_A R_{2,2} \bowtie_B R_{2,3} \text{ where}\\
%     & d_A(v,R_{1,1}) = 11\\
%     & d_A(v,R_{1,2}) = 6\\
%     & c_B(R_{1,2}) = 7\\
%     & c_B(R_{1,2}) = 10
% \end{align*}
% Then
% $$\mathcal{K}(v) = \min
% \left\{\begin{array}{l}
% 10 \cdot 9 \cdot 5\\
% 11 \cdot 6 \cdot 7\\
% \end{array}\right.$$

% To generalize for pairwise joins with different paths, if the first tables to be joined in two paths share same attribute $A$, we simply iterate through values in $C_A$ though they have different terms followed; if not, to be done... (can we iterate through a join attribute of an intermediate table in the join path?)

% \subsection{Naive Approach}
% \textbf{Case I: } Suppose $R_{1,1} \bowtie R_{1,2}$ and $R_{2,1} \bowtie R_{2,2}$ share the same join attribute(s), i.e. $A_{1,1} = A_{2,1}$. Let 
% $$\mathcal{C}_A = \mathcal{C}_{A_{1,1}}(R_{1,1}) \cap \mathcal{C}_{A_{1,1}}(R_{1,2}) \cap \mathcal{C}_{A_{2,1}}(R_{2,1}) \cap \mathcal{C}_{A_{2,1}}(R_{2,2})$$
% Then for each $v \in C_A$, we define
% \begin{align*}
%     \mathcal{K}(v) =
% &\min_{j\in\{1,2\}}\big\{d_A(v,R_{j,1}) \cdot  d_A(v,R_{j,2}) \cdot\\ &\min\{c_{A_{j,2}}(R_{j,2}),c_{A_{j,2}}(R_{j,3})\} \cdots \min\{c_{A_{j,n_j-1}}(R_{j,n_j-1}),c_{A_{j,2}}(R_{j,n_j})\big\}
% \end{align*}
% Then for an upper bound of $O_{12}$, we have
% $$O_{12} \leq \sum_{v\in C_A} \mathcal{K}(v)$$
% Notice that $\argmax_{v\in C_A} K(v) = \argmax d_A(v,R_{j,1}) \cdot  d_A(v,R_{j,2})$ since $\min\{c_A(R_{j,3}),c_B(R_{j,3})\}$ stays the same for all $v$. Hence if we define
% $$k(v) = \min_{j\in\{1,2\}}\{d_A(v,R_{j,1}) \cdot  d_A(v,R_{j,2})\}$$
% we have the equation rearranged as follows
% $$O_{12} \leq \sum_{v\in C_A} k(v) \cdot \prod_{i = 2}^{n_j-1} \min\{c_{A_{j,i}}(R_{j,i}),c_{A_{j,i}}(R_{j,i+1})\} \cdot$$

%Recall that $\mathcal{A}_j^k$ is the set of the tuples of $k$-th overlapped in join path $J_j$. Given $S = \{J_1, J_2,\dots, J_n\}$ where $J_j = R_{j,1} \bowtie_{A_1} R_{j,2} \bowtie_{A_2} \cdots \bowtie_{A_3} R_{j,n_1}$, let $\Delta$ be a subset of the powerset of $S$. Now we extend our value-based pair-wise overlapping estimation approach to find an upper bound for $\mathcal{O}_{\Delta_k}^k$ for any $k$.


\subsection{Overlap of Multiple Join Paths}
\label{sec:genericoverlap}

\fn{Now, we turn our attention to computing the overlap of multiple join paths. Let $\Delta$ be a set of join paths. We denote $J_j\in\Delta$ with $R_{j,1} \bowtie_{A_{j,1}} R_{j,2} \bowtie_{A_{j,2}} \cdots \bowtie_{A_{j,n_1-1}} R_{j,n_1}$. We make the same assumptions as pairwise overlaps.  That is, relations are unionable and the join attribute of the first two relations in all join paths are unionable. Let  $\mathcal{O}_{\Delta}= \vert \bigcap_{J_j\in\Delta}J_j \vert$ be the overlap of join paths in $\Delta$.}  
%Let $\mathcal{C} = \bigcap_{J_j\in\Delta} D_{A_1}(R{j,1} \cap D_{A_1}(R_{j,2})$. 
Let $\mathcal{C}=\bigcap_{J_j\in\Delta}\mathcal{D}_{A_{j,1}}(R_{j,1})\cap\mathcal{D}_{A_{j,2}}(R_{j,2})$. Following the idea that a loose bound for $\mathcal{O}_{\Delta}$ is $\min_{J_j\in\Delta}\{|J_j|\}$, for each $v \in\mathcal{C}$ we define
$$\mathcal{K}(v, 1) = \min_{J_j\in\Delta} \{d_A(v, R_{j,1}) \cdot d_A(v,R_{j,2})\}$$
which takes the minimum degree of value $v$ in all join paths in $\Delta$. Therefore, we have
the following. 
$$\mathcal{K}(1) = \sum_{v \in \mathcal{C}} \mathcal{K}(v,1)$$
Similarly, $\mathcal{K}(i)$ can be extended from the pairwise case.

\begin{theorem}
\label{ki}
Given a collection of join paths $S$ and a subset $\Delta\subset S$, let $O_{\Delta} = \bigcap_{J_j\in\Delta}J_j$ 
%where $|\Delta_k| = k$, denote $O_{\Delta_k}^k$ as 
be the set of tuples that appear in all $J_j \in \Delta$.  Let $M_{A_l}(R_{j,i})$ be  the maximum degree of values in the domain of a  join attribute $A_l$ of relation $R_{j,i}$ of join path $J_j$ and let  $d_{A_l}(v,R_{j,i})$ be the degree of value $v$ in the domain of $A_l$. We obtain an upper bound for $|O_{\Delta}|$ dynamically as follows. 
\begin{align*}
    |\mathcal{O}_{\Delta}| &\leq \mathcal{K}(n-1)\\
    &= \mathcal{K}(n-2) \cdot \min_{J_j\in\Delta}\{M_{A_{n-1}}(R_{j,n})\}
\end{align*}
where
\begin{align*}
    \mathcal{K}(1) &= \sum_{v \in \mathcal{C}} \mathcal{K}(v,1)\\
    &= \sum_{v\in\mathcal{C}}\min_{J_j\in\Delta}\{d_{A_1}(v,R_{j,1}) \cdot  d_{A_1}(v,R_{j,2})\}\\
    \mathcal{K}(i) &= \mathcal{K}(i-1) \cdot \min_{J_j\in\Delta}\{ M_{A_i}(R_{j,i+1})\}
\end{align*}
\end{theorem}
The proof for Theorem \ref{ki} can be extended from the deduction process discussed earlier. 
\fn{FN: how do we get values v and overlaps, etc.?}\yurong{yl: I assume that we are given information of degree of $v$'s}

\subsection{Overlap Estimation: General Case}
\label{sec:overlapgeneral}

\fn{So far, we proposed a way of estimating the overlap of multiple join paths of the same length where for each relation $R_{j,i}$ in $J_j$ there is a corresponding unionable relation with the same number of attributes in each of other join paths.}
We now release this assumption \fn{to accommodate join paths with arbitrary size and arbitrary relation schemas. Note that the join paths themselves should still have the same schemas after join.} 
%that each chain join path $J_j$ has same structure and length 
We introduce the ``splitting method''  \fn{that derives new join paths by breaking down  relations into sub-relations, each sub-relation consisting of exactly two attributes. The derived  join paths all have the same schema, each generate the same data as the original path, and all contain the same number of relations. Moreover, for each relation in a derived join path, there are corresponding unionable relations in other join paths. Since, the derived join paths satisfy the requirements of \S~\ref{sec:overlapgeneral} and generate the same data, we can directly apply Theorem~\ref{ki} to estimate the overlap size of the original join paths.   
%Note that the key \dn{idea} here is 
%Although the derived join paths have different relations, the schema of the resulting table will be the same after performing full joins. 
Although the input join paths may not include unionable relations, they definitely have  unionable attributes and the same schema after join. 
As such, breaking all relations in sub-relations of two attributes and redefining join paths incurs join paths with the same number of relations and unionable relations. Note that our splitting method is different than the normalization in the database theory which aims to decompose relations into sub-relations based on functional dependencies to avoid anomalies~\cite{Codd71a}.} 

\fn{For simplicity, we rename unionable attributes of join paths to have the same unique names. For example, in the join paths of  Table~\ref{tab:splitjoin}, attributes labeled with $A$ are all unionable and different than attributes labeled with $B$. Then, attributes of each relation are organized based on the lexicographical ordering. Next, a relation $R_{i}$, with $m$ attributes, in join path $J$, is split into a derived join path of two-attribute relations $R_{i,1}\bowtie^\prime R_{i,2}\cdots\bowtie^\prime R_{i,m-1}$, where $R_{i,k}$ is a relation consisting of the $k$th and $k+1$th attributes of $R_{i}$. Here, to avoid generating spurious tuples when computing the overlap and join, 
%$\bowtie^\prime$ strictly indicates that each tuple is only joined with one other tuple. 
we redefine the ``join'' performed on $R_{i,j}$'s. The operation    $\bowtie^\prime$, also referred as ``fake join'',  in  $R_{i,1}\bowtie^\prime R_{i,2}\cdots\bowtie^\prime R_{i,m-1}$  is a  natural join and is defined such that  $R_{i,j}$ and $R_{i,j+1}$ have a one-to-one relationship between tuples in join attributes. That is, $|R_{i,1}\bowtie^\prime R_{i,2}\cdots\bowtie^\prime R_{i,m-1}| = |J|$. }


\begin{example} In Table \ref{tab:splitjoin}, paths $J_1, J_2$ and $J_3$  all have the same schema with attributes $A,B,C,D,E$. However, relations in each path originally have different attributes.  The split method decomposes each join path into two-attribute-relation chain joins shown in Table~\ref{tab:splitjoin}. When splitting a relation with attributes $(A,B,C)$ to relations $(A,B)$ and $(B,C)$, we split each tuple $t(A,B,C)$ into $t(A,B)$ and $t(B,C)$ with the same value on $B$, hence, $(A,B)$ and $(B,C)$ always have a one-to-one relationship for the same tuple. We also redefine the ``join'' performed on such $(A,B)$ and $(B,C)$. For example, in $J_1$, the join  $(B,C) \bowtie (C,D)$ represents a ``real'' join connecting the first two relations of the path. However, $(A,B) \bowtie^\prime (B,C)$ represents a ``fake'' join connecting tuples of one relation. \fn{FN: can you double check the next few sentences. Hard to understand.} \yurong{(yl: the following sentences  are used to explain the method we use to calculate the number of resulting tuples we'll get after the fake join )} Suppose $(A,B) \bowtie^\prime (B,C)$ is performed \yurong{as the first join in a join path as in $J_1$. Since $(A,B)$ wasn't joined with other tables and remains the same,} the resulting relation will be exactly the original relation $(A,B,C)$ so $|(A,B)| = |(B,C)| = (A,B,C)|$. Now, if we look into $J_2$ where the ``fake'' join is performed on $(A,B,C)$ \yurong{(since we have $(B,C)$ joined with $(A,B)$)} and $(C,D)$, in order to reproduce the tuples in the original relation without generating bogus tuples, we follow the one-to-one property that each tuple $t$ in  $(A,B,C)$ can only be mapped to one tuple with $t.C$ on attribute $C$ in relation  $(C,D)$. Hence, $|(A,B,C) \bowtie^\prime (C,D)| = |(A,B,C)|$. %\yurong{yl: please let me know if this sounds clear} 
Note that $J_3$ can also be decomposed into the same form as $J_1$ and $J_2$ since order of tables doesn't matter in chain join. We could randomly choose a standard form of normalization for all the join paths. \yurong{(or we could come up with a trick to find a best(most common) order)}
\fn{FN: what do you mean here?} \yurong{yl: how we define the standard order of joins on sub-relations}
\end{example}


%In order to apply the split method to estimate the overlapping information in this general case, we want to each table in each join path become unionable with other corresponding. 
%We now explain (3) in detail. 

After the normalization, we derive a corollary for Theorem \ref{ki} to estimate $O$'s in the general case.
\begin{corollary}
\label{ki}
Given a collection of split join paths $S$ and a subset $\Delta\subset S$, let $O_{\Delta} = \bigcap_{J_j\in\Delta}J_j$ 
%where $|\Delta_k| = k$, denote $O_{\Delta_k}^k$ as 
be the set of tuples that appear in all $J_j \in \Delta$.  Let $M_{A_l}(R_{j,i})$ be  the maximum degree of values in the domain of a  join attribute $A_l$ of relation $R_{j,i}$ of join path $J_j$ and let  $d_{A_l}(v,R_{j,i})$ be the degree of value $v$ in the domain of $A_l$. Define
\begin{align*}
    M_{j,i} = \left\{\begin{array}{l}
    M_{A_i}(R_{j,i+1})\; \text{ if }\;  R_{j,i} \bowtie R_{j,i+1}\\
    \\
    |R_{j,i}|\; \text{ if }\; R_{j,i} \bowtie' R_{j,i+1}
\end{array}\right.
\end{align*}
We then obtain an upper bound for $|O_{\Delta}|$ dynamically as follows. 
\begin{align*}
    |\mathcal{O}_{\Delta}| &\leq \mathcal{K}(n-1)\\
    &= \mathcal{K}(n-2) \cdot
    \min_{J_j\in\Delta}\{M_{j,n}\}
\end{align*}
where
\begin{align*}
    \mathcal{K}(1) &= \sum_{v \in \mathcal{C}} \mathcal{K}(v,1)\\
    &= \sum_{v\in\mathcal{C}}\min_{J_j\in\Delta}\{d_{A_1}(v,R_{j,1}) \cdot  d_{A_1}(v,R_{j,2})\}\\
    \mathcal{K}(i) &= \mathcal{K}(i-1) \cdot \min_{J_j\in\Delta}\{ M_{j,i}\}
\end{align*}
\end{corollary}

\begin{table}[]
\small
    \centering
    \begingroup
    \setlength{\tabcolsep}{1.5pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.5} % Default value: 1
    \begin{tabular}{ll}
    $J_1 = (A,B,C) \bowtie (C,D,E)$ & $\Rightarrow (A,B) \bowtie' (B,C) \bowtie (C,D) \bowtie' (D,E)$\\
    $J_2 = (A,B) \bowtie (B,C,D) \bowtie (D,E)$ & $\Rightarrow (A,B) \bowtie (B,C) \bowtie' (C,D) \bowtie (D,E)$\\
    $J_3 = (B,C) \bowtie (A,B,D,E)$ & $\Rightarrow (A,B) \bowtie (B,C) \bowtie' (C,D) \bowtie' (D,E)$\\
    \end{tabular}
    \endgroup
    \caption{Example of splitting method}
    \label{tab:splitjoin}
\end{table}

\subsection{$k$-Overlap of Join Path} 
\label{sec:koverlap}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figs/koverlap.jpg}
    \vspace{-5mm}
    \caption{Computing $\mathcal{A}_j^k$ using pairwise overlap.}
    \label{fig:koverlap}
\end{figure}

% \paragraph{Theorem x} Let $S = \{J_1, J_2, J_n\}$, and $\Delta$ be a subset of the powerset of $S$. Let $B = \binom{n}{n-(k-1)}$, then for any join path $J_j$, and xfor any $k$ from $1$ to $n$, we have
% $$A_j^k = \sum_{j \in \Delta} O_{\Delta}^k - \binom{n}{k-1} \big(\frac{n-1}{B} A_j^n + \frac{n-2}{B} A_j^{n-1} + \frac{n-3}{B} A_j^{n-2} + \cdots \frac{k}{B} A_j^{k+1} \big).$$
% Thus when $k = n$,
% $$A_j^n = \sum_{j \in \Delta} O_\Delta^5,$$
% and when $k = 1$
% $$A_j^1 = \sum_{j \in \Delta} O_\Delta^1 - \sum_{k = 2}^n A_j^k = |J_j| - \sum_{k = 2}^n A_j^k.$$
%With information of $\mathcal{O}_{\Delta_k}^k$, we now have a theorem for calculating $A_j^k$ dynamically for each $j$ and $k$.

\subsection{Computing $\mathcal{A}$}

\fn{Having described a way of computing the overlap for any subset $k$ of join paths, $\mathcal{O}_{\Delta}$, we turn our attention to computing the part of a join path $J_j$ that appears in exactly $k$ join paths, $\mathcal{A}_j^k$. }

\begin{example} \label{ex:koverlap} 
\fn{Consider the join paths $J_1, \cdots, J_4$ of Figure~\ref{fig:koverlap}. The areas $\mathcal{A}_1^k$ for $k\in[1,4]$ are color-coded. Clearly, $\mathcal{A}_1^4$ is equivalent to $\mathcal{O}_S$, whose size we already have a way of computing. Suppose we would like to compute $|\mathcal{A}_1^2|$. 
Note that the total sum of the size of dotted, +, and x areas indicates the sum of the pairwise overlap of join paths, i.e., $\sum_{\Delta\in P_2\wedge J-1\in P2}|\mathcal{O}_{\Delta}|$. However, to determine $\mathcal{A}_1^2$, we need to exclude all $\mathcal{A}_1^3$ and $\mathcal{A}_1^4$ areas. In fact, each subarea of $\mathcal{A}_1^3$ counts twice in $|\mathcal{A}_1^2|$. For example, $J_1\cap J_2\cap J_3$ is in both $J_1\cap J_2$ and $J_1\cap J_3$. Similarly, $\mathcal{A}_1^4$ counts three times in the sum of $\mathcal{O}_{\Delta}$'s since it is included in $J_1\cap J_2\cap J_3$, $J_1\cap J_2\cap J_4$, and $J_1\cap J_3\cap J_4$. } 
\end{example}

Using the intuition explained in Example~\ref{ex:koverlap}, we now introduce a theorem for computing $\mathcal{A}_j^k$. 

\begin{theorem}
\label{Ajk}
Let $S = \{J_1, J_2, \dots J_n\}$ \fn{and $P_k$ be the set of all subsets of size $k$ of $S$, } 
%and $\Delta_k$ be a subset of the powerset of $S$ of size $k$, 
then for any join path $J_j$, and for any $k$ from $1$ to $n$, we have
%$$|\mathcal{A}_j^k| = \sum_{J_j \in \Delta_k} |\mathcal{O}_{\Delta_k}^k| - ( \sum_{r=k+1}^{n} \binom{r-1}{k-1} \cdot |\mathcal{A}_j^{r}| ).$$

$$|\mathcal{A}_j^k| = \sum_{\Delta\in P_k\wedge J_j} |\mathcal{O}_{\Delta}| - ( \sum_{r=k+1}^{n} \binom{r-1}{k-1} \cdot |\mathcal{A}_j^{r}|).$$
For $k = n$ we have 
%$$|\mathcal{A}_j^n| = \sum_{J_j \in \Delta_n} |\mathcal{O}_{\Delta_n}^n| = |\mathcal{O}_{S}^n|,$$
\fn{$$|\mathcal{A}_j^n| = |\mathcal{O}_{S}|,$$}
%\sum_{\Delta\in P_n\wedge J_j \in P_n} |\mathcal{O}_{\Delta}| = |\mathcal{O}_{S}|,$$}
% fn not sure we need the case of k=1
\eat{
For $k = 1$ we have 
%$$|\mathcal{A}_j^1| = \sum_{J_j \in \Delta_1} |\mathcal{O}_{\Delta_1}^1| - \sum_{r = 2}^{n} \binom{r-1}{0} |\mathcal{A}_j^k| = |J_j| - \sum_{r = 2}^n |\mathcal{A}_j^r|.$$
\fn{$$|\mathcal{A}_j^1| = \sum_{\Delta\in P_1\wedge J_j \in P_1} |\mathcal{O}_{\Delta}| - \sum_{r = 2}^{n} \binom{r-1}{0} |\mathcal{A}_j^k| = |J_j| - \sum_{r = 2}^n |\mathcal{A}_j^r|.$$}
}
\end{theorem} 
\begin{proof}
%When $k = n$, $\mathcal{O}_{\Delta_n}^n$ represents the overlap of all $n$ join paths in $S$, i.e. $\bigcap_{J_j \in S} J_j$. In this case, $\Delta_n$ contains all $n$ join paths and hence is the universe $S$, thus it's trivial that the $n$-th overlap $|\mathcal{A}_j^n| = |\mathcal{O}_{S}^n|$ for any join path $J_j$. 
\fn{When $k = n$, $P_n$ is one set representing the universe $S$ including $J_j$. Therefore, it is trivial that  
$|\mathcal{A}_j^n| = O_S$, which can be evaluated 
with $\bigcap_{J_j \in S} J_j$.} Then, for $k \in [2, n-1] \cap \mathbf{Z}$, we calculate $|\mathcal{A}_j^k|$ dynamically. 
\fn{Now, suppose we know $|\mathcal{A}_j^{k+1}|$. 
Recall $\mathcal{A}_j^k$ consists of all tuples in $J_j$ that appear in exactly $k-1$ other join paths. That is, tuples in $J_j$ that are in some $\Delta\in P_k$ but are not in any higher order overlap  $\Delta^\prime\in P_{r}$, where $r\in[k+1,n]$. 
Therefore, we first add up all the $k$-th overlap for sets $\Delta\in P_k$ where $J_j \in \Delta$.
Since $J_j$ is confirmed, we have $\binom{n-1}{k-1}$ number of such sets $\Delta$. 
Note that a tuple $t\in\mathcal{A}_j^k$ may appear in multiple $\Delta\in P_r, r\in[k+1,n]$. 
Therefore, to get the exact value of $|\mathcal{A}_j^k|$, 
for each $r\in[k+1,n]$, 
we need to count the number of $\Delta\in P_r$ where $J_j\in\Delta$. 
Starting with $r = k+1$, each such combination of $\Delta\in P_{k+1}$ contains $J_j$, therefore, it  appears once in remaining $\binom{k}{k-1}$ number of $\Delta^\prime\in P{k}$'s. 
Hence, we need to deduct $(k-1)\cdot |\mathcal{A}_j^{k+1}|$ from the sum. 
For example, if $\Delta=\{J_1, J_2, J_3, J_4\}$ and $j=1$, we have $\Delta$ appearing in $\{J_1, J_2, J_3\}$, $\{J_1, J_2, J_4\}$, and $\{J_1, J_3, J_4\}$ combinations, which are all in $\mathcal{A}_1^3$. 
Now for the general case $r$, where $k < r\leq n$, after $J_j$ is confirmed, each combination of $\Delta\in P_r$ has its other $k-1$ paths chosen in $\binom{r-1}{k-1}$ number of $\Delta^\prime\in P_{k}$, so a total number of $\binom{r-1}{k-1}$ $|\mathcal{A}_j^{r}|$ needs to be deducted from the sum for each $r$. 
}
\eat{
We first add up all the $k$-th overlap for sets $\Delta_k$ where $J_j \in \Delta_k$. Since $J_j$ is confirmed, we have $\binom{n-1}{k-1}$ number of such $\Delta_k$. Then we want to know how many times $|\mathcal{A}_j^{r}|$ which are information we've gained earlier, where $k < r \leq n$, are counted in this sum. Starting with $r = k+1$, each combination of $\Delta_{k+1}$ appears once in $\binom{k}{k-1}$ number of $\Delta_{k}$'s, as $J_j$ is confirmed, and we only have $\binom{1}{k+1-k} = 1$ path left after other $k-1$ paths are chosen. Hence we need to deduct $(k-1)\cdot |\mathcal{A}_j^{k+1}|$ from the sum. Now for the general case $r$ where $k < r\leq n$, after $J_j$ is confirmed, each combination of $\Delta_{r}$ has its other $k-1$ paths chosen in $\binom{r-1}{k-1}$ number of $\Delta_{k}$'s, so a total number of $\binom{r-1}{k-1}$ $|\mathcal{A}_j^{r}|$'s needs to be deducted from the sum for each $r$. To further illustrate the idea, we then take $r = n$ as an example. Notice that the overall overlap $\mathcal{A}_j^n$ is counted once in every $\Delta_k$, so we need to subtract $\binom{n-1}{k-1} \cdot |\mathcal{A}_j^n|$ from the sum. }
Therefore, we can organize the formula of calculating $|A_j^k|$ as shown in the theorem. 
%$$|\mathcal{A}_j^k| = \sum_{J_j \in \Delta_k} |\mathcal{O}_{\Delta_k}^k| - ( \sum_{r=k+1}^{n} \binom{r-1}{k-1} \cdot |\mathcal{A}_j^{r}| )$$
\end{proof}

\fn{Using this theorem to calculate $|A_j^k|$'s for a given $J_j$ and all $k\in[1,n]$, we start by initializing $|A_j^n|$ with $|\mathcal{O}_S|$ using the method proposed in \S~\ref{sec:genericoverlap}. Then, $|A_j^{n-1}|$ requires evaluating $|A_j^n|$ that have been already computed as well as $|\mathcal{O}_{\Deltal}|$ for each subset of size $n-1$ of $S$. 
Again, \S~\ref{sec:genericoverlap} is used to compute a $|\mathcal{O}_{\Deltal}|$. In general, iterating from $n-1$ to $1$, each $|A_j^k|$ can be computed from $|A_j^r|$'s, where $r\in(k,n]$, that have been already evaluated and $|\mathcal{O}_{\Deltal}|$'s that can be computed from our method for the pairwise join path overlap.}

\fn{FN: explain the complexity of this method. do you think we need an pseudo code or it is clear?} 

\eat{
\section{Hashing Approach (Needs revisiting)}
\label{sec:samplejoin}

The random sampling framework raised in \cite{2018_sample_join_revisit} relies on efficient access to the underlying data, and hence requires complete index structures when going from one relation to another during the join process. In order to extend the usage of our framework beyond in-memory database where index structures are often built, we introduce the hashing approach when performing actual joins. We start with the binary case.\\
\textbf{Binary case.} 
Let $J_j = R_1 \bowtie_{A_1} R_2$. For table $R_1$ and $R_2$, let $A_1$ be the set of join attributes. Then we hash table $R_1$ and $R_2$ on attributes in $A_1$.
% \textcolor{blue}{Let tuples in $R_1$ be $t_1^1, t_1^2, \dots, t_1^n$, and tuples in $R_2$ be $t_2^1, t_2^2, \dots, t_2^m$. Then we define a hash function $h$ such that
% $$h(t_1^i) = h(t_2^j) \Leftrightarrow \pi_B(t_1^i) = \pi_b(t_2^j)$$}
% Let $h:\mathcal{A_1} \rightarrow [0,1]$ be a hash function that uniformly maps the join values into range $[0,1]$.\\
Suppose the tuples from the two tables are hashed into $n$ buckets, and the buckets are uniformly distributed. Thus we have the probability of selecting each bucket $b_k$ as
$$P(b_k) = \frac{1}{n}$$
% \textcolor{blue}{Let $d_B(t,R_i)$ denote the degree of value $t$ in $R_i$, then we define the probabilities
% \begin{align*}
%     P(t_1^i) &= \frac{1}{d_B(\pi_B(t_1^i),R_1)}\\
%     P(t_2^j) &= \frac{1}{d_B(\pi_B(t_2^j),R_2)}
% \end{align*}}
Let $b_i^k$ denote the bucket of $R_i$ with index $k$, and $b_{i,u}^k$ denote the bucket of $R_i$ that contains value $u$. Then we have the probability of selecting $t_{i,u}$ from its bucket as
$$P(t_{i,u}) = \frac{1}{|b_{i,u}^k|}$$
Now note that since we are not doing perfect hashing, after randomly selecting $t_{1,a}$, there's possibility that $t_{2,u}$ randomly chosen from $b_{2,u}^{k'}$ does not satisfy $u = a$. In this case, $t_{1,a}$ and $t_{2,u}$ can't be joined together. In order to guarantee independence, if $t_{2,u}$ can be joined with $t_{1,a}$, we accept $t_{2,u} = t_{2,a}$ and continue; but if not, $t_{2,u}$ is rejected, then we abandon $t_{1,a}$ and start from the first step of sampling. Hence, we have the probability of selecting $t_{2,a}$ as
\begin{align*}
    P(t_{2,a} \mid t_{1,a}) &= \frac{\frac{1}{n}\cdot \frac{1}{|b_{1,a}^k|}\cdot\frac{1}{d_{A_1}(a,R_2)}}{\frac{1}{n}\cdot \frac{1}{|b_{1,a}^k|}}\\
    &= \frac{1}{d_{A_1}(a,R_2)}
\end{align*}
Then to satisfy the uniform requirement, we want the probability of selecting any joined sample to be $$P(t_1 \bowtie t_2) = \frac{1}{|J_i|}$$
Hence the acceptance rate is
% $$\frac{\frac{1}{|\Tilde{J}|}}{ \frac{1}{n} \cdot P(t_{1,u}) \cdot P(t_{2,u})} = \frac{n \cdot |b_{1,u}^k| \cdot |b_{2,u}^{k'}|}{|\Tilde{J}|}$$
% \begin{align*}
%     \frac{\frac{1}{|J_j|}}{\frac{1}{n} \cdot P(t_{1,u}) \cdot P(t_{2,u})} &= \frac{n \cdot |b_{1,u}^k| \cdot d_{A_1}(a,R_2)}{P(J_j)\cdot |U|}\\
%     &= \frac{|U| \cdot n \cdot |b_{1,u}^k| \cdot d_{A_1}(a,R_2)}{|J_j|\cdot |U|}\\
%     &= \frac{n \cdot |b_{1,u}^k| \cdot d_{A_1}(a,R_2)}{|J_j|}
% \end{align*}
$$ \frac{\frac{1}{|J_j|}}{\frac{1}{n} \cdot P(t_{1,u}) \cdot P(t_{2,u})} = \frac{n \cdot |b_{1,u}^k| \cdot d_{A_1}(a,R_2)}{|J_j|}$$

\textbf{General case.}
For the general case, we do hashing on the join attribute for each table in the full join path based on the first pairwise join it's involved. For example, if $J_j = R_1 \bowtie_{A_1} R_2 \bowtie_{A_2} R_3$, we only hash tuples from $R_1$ on attributes $A_1$, tuples from $R_2$ on attributes $A_1$, and tuples from $R_3$ on attributes $A_2$. We'll explain the reason behind this idea in further sampling steps.\\
There are two ways of sampling after hashing, the only difference is on the first step.\\ 
When we sample a tuple $t_{1,a}$ from $R_1$, we have two choices. One way is to randomly select a tuple directly from $R_1$ with probability $\frac{1}{|R_1|}$; the other way is first randomly choose a bucket $b_1^k$ with probability $\frac{1}{n}$, and then randomly sample a tuple from the selected bucket with probability $\frac{1}{|b_1^k|}$. The following steps will all be the same.\\
After $t_{1,a_1}$ is selected, we randomly choose a $t_{2,u}$ from the corresponding bucket $b_{2,a}^{j_2}$ for $R_2$. Similar to the binary case, in order to guarantee independence, in any step of sampling tuples followed, if $t_{i,u}$ can be joined with $t_{i-1,a}$, we accept $t_{i,u}$ and continue; but if $t_{i,u}$ is rejected, we abandon all $t_{l,a}$ where $l < i$ and start from the first step of sampling. Assume $t_{2,a_1}$ is accepted, we then hash $t_{2,a_2} = t_{2,a_1}$ on attribute $A_2$, and go to the bucket $b_{2,a_2}^{k_3}$. Similarly, we randomly choose $t_{3,u}$ from $b_{2,a_2}^{k_3}$. In this case, the final acceptance rate is 
$$\frac{|R_1| \cdot |b_{2,a_1}^{k_2}| \cdot |b_{3,a_2}^{k_3}|}{|J_j|}$$
or if using the second approach
$$\frac{n \cdot |b_{1,a_1}^k| \cdot |b_{2,a_2}^{k_2}| \cdot b_{3,a_2}^{k_3}|}{|J_j|}$$
\textcolor{blue}{(Mention difference with Ripple Join (not independent)}\\
\textcolor{blue}{Hash table memory}

% \subsection{Sampling Methods}
% \textbf{Estimating Join Size by Correlated Sampling}\\
% \textbf{two-table} 
% Correlated sampling\cite{cor_sampling} employs hashing method to generate correlated samples which helps handle the join relationship between two tables while sampling. The idea of correlated sampling in two table case is as follows.\\ 
% Suppose we want to estimate the size of $J = R_1 \bowtie R_2$ which join on values from the join attribute(s) which is formed as a set $\mathcal{V}$. Let $h:V \rightarrow [0,1]$ be a hash function that uniformly maps the join values into range $[0,1]$. Let $p$ be the sampling probability. Then for every sampled tuple $t_v$ (with value $v$), it's accepted if $h(v) < p$. In this way, a pair of tuples that could be joined share the same join value and thus will both be accepted with probability $p$, and be rejected with probability $1-p$. Let the sample of $R_1$ and $R_2$ be $S_1$ and $S_2$. We can then compute the size of the joined sample and scale it up by $p$, and hence the estimated join size $|\Tilde{J}| = \frac{|S_1 \bowtie S_2|}{p}$.\\
% \textbf{multi-table}\\

% \noindent \textbf{Estimating Overlap by Sampling with Hashing}
% We want to continue to use the hashing and sampling method for join size estimation for overlapping size estimation.\\
% General Idea: For $J_1$ and $J_2$, we obtain set of samples when estimating their sizes, say $\Gamma_1 \subset J_1$ and $\Gamma_2 \subset J_2$, where $|\Gamma_1| = |\Gamma_2|$. Let the overlapping part $O_{\Gamma_{12}} = \Gamma_1 \cap \Gamma_2$, then since
% $$\frac{|J_1 \cap J_2|}{|J_1| + |J_2|} = \frac{|\Gamma_1 \cap \Gamma_2|}{|\Gamma_1| + |\Gamma_1|}$$
% (This is the general idea which is not verified yet. Maybe it's not pluls on the denominater. Need to first guarantee iid, calculate probabilities and variance analysis)
% we propose that the estimated pairwise overlapping size between $J_1$ and $J_2$ is
% $$O_{12} = |J_1 \cap J_2| = \frac{|O_{\Gamma_{12}}| \cdot (|J_1| + |J_2|)}{|\Gamma_1| + |\Gamma_1|}$$


% \noindent \textbf{High Level Idea}
% Since both the join size estimation step and sampling step needs hashing, we can just perform it one time. The high level idea is that we can use the samples from the size estimation step and guarantee I.I.D. at the same time (which can be extremely difficult to compute).
}

==> apendix.tex <==
% \section{Appendix}

% \begin{definition} {\em{\bf (Distribution-Preserving Union of Joins Sampling)}} Given join paths $S = \{J_1, \ldots, J_n\}$, where each join path is a chain of relations $J_i = R_{i1}\bowtie\ldots\bowtie R_{im}$. Each $J_i$ is sampled from a probability distribution $\theta$, then we return $N$ independent samples $T=\{t_1,\cdots,t_n\}$, such that $T$ subjects to $\theta$.
% \end{definition}

% \begin{algorithm}
% \caption{Exact Distribution-Preserving Union of Joins Sampling}
% \begin{small}
% \begin{algorithmic}[1]
% \Require{Join paths $S = \{J_j, 1\ \leq j \leq n\}$, Tuple count $N$}
% \Ensure{Tuples $\{t_i, 1 \leq i \leq N\}$}
% \State $S \leftarrow \{\}$ \Comment{target sample}
% \For{j = 1,2,\dots, n}
% \State Calculate $|J_j|$ 
% \EndFor
% \For{k = 1,2,\dots, n}
% \For{each power set $\Delta_k$ of $S$}
% \State Calculate $O^k_{\Delta_k}$ 
% \EndFor
% \For{j = 1,2,\dots, n}
% \State Calculate $A_j^k$
% \EndFor
% \EndFor
% \While{$n < N$}
% \State $J \leftarrow$ a random join path $J_j$ with probability $\frac{\sum_{k=1}^n\frac{1}{k}A_j^k}{|J_1\cup\cdots\cup J_n|}$
% \State $t \leftarrow$ a sample from $J$ using hashing approach
% \State add $t$ to $S$
% \State $n \leftarrow n + 1$
% \EndWhile
% \State \textbf{return} $S$
% \end{algorithmic}
% \end{small}
% \end{algorithm}

% \begin{algorithm}
% \caption{Fast Distribution-Preserving Union of Joins Sampling}
% \begin{small}
% \begin{algorithmic}[1]
% \Require{Join paths $S = \{J_j, 1\ \leq j \leq n\}$, Tuple count $N$}
% \Ensure{Tuples $\{t_i, 1 \leq i \leq N\}$}
% \State $S \leftarrow \{\}$ \Comment{target sample}
% \For{i = 1,2,\dots, n}
% \State Calculate $|J_i|$ 
% \For{j = i,i+1,\dots, n}
% \State Calculate $O_{ij}$ 
% \EndFor
% \State $A_i^1 = |J_i| - \max_{j}O_{ij}$ 
% \EndFor
% \While{$n < N$}
% \State $J \leftarrow$ a random join path $J_i$ with probability $\frac{2A_i^1+\sum_{k} O_{ik}}{ 2\sum_i A_i^1 +\sum_{i} \sum_{k} O_{ik}}$
% \State $t \leftarrow$ a sample from $J$ using hashing approach
% \State add $t$ to $S$
% \State $n \leftarrow n + 1$
% \EndWhile
% \State \textbf{return} $S$
% \end{algorithmic}
% \end{small}
% \end{algorithm}

==> complexity.tex <==
\section{Complexity Analysis}
\label{sec:complexity}



\textcolor{red}
{In this section, we discuss the time complexity analysis of Algorithm \ref{alg1}, \ref{algB}, and \ref{algNB}. 
Let the time of sampling from a single join path be $t$ following the method proposed by \citet{2018_sample_join_revisit}, the target number of samples be $N$, and the number of join paths be $m$. Note that in set union sampling, some iteration rejects the tuple if it's not from the assigned join path. We define the delay between two successful answers as $D$ for now and will provide a full analysis of it in our future work.
\subsubsection*{Disjoint Union of Joins Sampling}
Since every tuple successfully returned by sampling over a single join \citet{2018_sample_join_revisit} is accepted, the runtime of Algorithm \ref{alg1} is simply $O(N \cdot t)$
\subsubsection*{Bernoulli Set Union Sampling}
In each round, we first iterate over all the join paths, and in the worst case, we need to select a tuple from each of them. Since we need to keep track of the $round\_recs$, whose size is bounded by $m$, and iterate over it to ensure uniformity, we have that each round has runtime $O(m^2\cdot t)$. We let the upper bound of the number of iterations be $N + c$, where $c$ is a constant obtained from the analysis on the last few rounds, which we will also conduct in the future. In addition to those, other operations can all be done in constant time. Together, we have the runtime for Algorithm \ref{algB} be $O((N+c) \cdot m^2 \cdot t \cdot D)$
\subsubsection*{Non-Bernoulli Set Union Sampling}
The Non-Bernoulli case is simpler. Within $N$ rounds, we sample a tuple with time $t$ from the selected join path. Aside from it, other operations can all be done in constant time. Hence considering the delay between accepted tuples, the runtime for Algorithm \ref{algNB} is $O(N\cdot t \cdot D)$
}

==> disjointunion.tex <==
\section{Sampling Disjoint Union}
\label{sec:disjointunion}

\todo{removed the pesuedo and moved some text to the previous section}.  

\eat{
We first solve the disjoint union case which is simpler. Algorithm~\ref{alg1} shows the pseudocode for sampling a disjoint union. Given the disjoint union $V = J_1\uplus\ldots\uplus J_n$,  we first select a join path $J_j$ with probability $P(J_j) = \frac{|J_j|}{|J_1+\ldots+J_n|}$, then, we  select a random tuple from $J_j$. We repeat the process until $N$ sampled tuples are obtained. 

\begin{algorithm}
\caption{Disjoint Union of Joins Sampling}
\begin{small}
\begin{algorithmic}[1]
\Require{Join paths $S = \{J_j, 1\ \leq j \leq n\}$, Tuple count $N$, join path sizes  $\{|J_j|, 1\ \leq j \leq n\}$,}
\Ensure{Sample $T = \{t_i, 1 \leq i \leq N\}$}
\State $\{|J_j|, 1\ \leq j \leq n\} \leftarrow warmup(S)$
\Comment{direct (\S~\ref{sec:joinsize}) or online (\S~\ref{sec:onlinejoinsize})}
\State $T \leftarrow \{\}$
\Comment{target sample}
\While{$n < N$}
\State $J \leftarrow$ a random join path $J_j$ with probability $\frac{|J_j|}{\sum_{j=1}^n |J_j|}$
\State $t \leftarrow$ sample from  $J$, add $t$ to $T$, $n \leftarrow n + 1$ 
\Comment{using  \S~\ref{sec:samplingjoin}}
%\State add $t$ to $T$, $n \leftarrow n + 1$
\EndWhile
\State \textbf{return} $T$
\end{algorithmic}
\label{alg1}
\end{small}
\end{algorithm}

Methods of sampling a tuple from a single join path has long been a popular problem~\cite{Olken,Chaudhuri:1999,2018_sample_join_revisit,viswanath1998join,Chaudhuri:1999}. We revisit random sampling over join in \S~\ref{sec:samplingjoin}.  


\begin{theorem}\label{th:disunionsampling}
Given join paths $S=\{J_1,\ldots, J_n\}$, Algorithm~\ref{alg1} returns each result tuple $t$ with probability $\frac{1}{|J_1+\ldots+J_n|}$. 
\end{theorem}
\begin{proof} The algorithm selects join path $J_j$ is selected with probability $|J_j|/|V|$ and a tuple $t$ in $J_j$ has probability $1/|J_j|$ of being selected at random. Therefore, we have $P(t) = \frac{|J_j|}{|V|} \cdot \frac{1}{|J_j|} = \frac{1}{|V|}$. 
%\begin{align*} 
%     P(t) = \frac{|J_j|}{|V|} \cdot \frac{1}{|J_j|} = \frac{1}{|V|}
%\end{align*}
\end{proof}

Algorithm~\ref{alg1} always returns independent samples because a returned sample is always uniform regardless of the previous sampling iterations. In order to calculate the probability distribution of join paths, we need to estimate $|J_j|$ for all $j$'s, during the pre-processing phase. There are various  ways of upper bounding the size of a join of two relations in the database theory community~\cite{ngo2018worst}.  
Regardless of the choice of algorithms for join estimation and random sampling over join, Algorithm~\ref{alg1} always returns independent samples since the returned sample is always uniform regardless of the history of samples. 
}


==> intro_bkup.tex <==
\section{Introduction}
\label{sec:intro}

\eat{Relational database (RDBMS) is a type of database which allows users to identify and access data in relation to another piece of data in the database. Data in a relational database is often organized into tables. Therefore, not only does the data themselves are stored, but also the relations between them are accessible in a database. The join operation is one of the basic query operations for relational databases which plays an important role in RDBMS, which is a  process that facilitates the retrieval of information about two different relations based on all possible combinations of rows of the two tables. Joins are frequently performed in real life. For instance, stores like Walmart may find the patterns for goods that usually being bought by a customer simultaneously, then it can put these goods together so customers would feel convenient or they may be reminded of the related things they have to purchase. In this scenario, Walmart could join the tables to achieve information of goods being bought by each customer. Additionally, AI and machine learning are compared with relational databases from an evolutionary perspective nowadays. \citet{mldb} describe the significant advantages of combining data processing with modeling optimization problems within databases in common machine learning algorithm usage scenarios. Some powerful Unified systems such as Spark also integrates relational algebra with high-level machine learning algorithms. Nevertheless, join is computationally expensive, especially over entire contents of large amounts of data and multiple relations. What's more, the unsophisticated implementations in typical big data environments make join even more expensive, and the lack of effective parallelization for those implementations means that we can't optimize simply by adding more hardware. Because the space complexity is also quadratic, large joins often run out of memory and need to be stored on disk which makes processing even slower.} 



Data scientists often draw on multiple sources during the data collection process~\cite{}. % citation to data centric AI
Since, most relational sources are not stored as single tables due to normalization, data scientists often need to perform joins before learning on the join output. Moreover, data may be collected from distributed sources, each described as a join over internal databases,  data lakes, or web data~\cite{AsudehN22,ChepurkoMZFKK20}. Therefore, the data is the  union of the  results of joins. 


Because joins are expensive to compute and learning after joins leads to poor training performance due to the introduced 
redundancy avoided by normalization, there has been efforts in 
enabling learning over joins, but they are limited to   certain models, including gradient descent with linear regression and cannot be applied to more general models~\cite{KumarNP15,KumarNPZ16,SchleichOC16,ChenKNP17}. 
Fortunately, an important result from the learning theory states that the sample size needed to train a model up to a $(\delta,\epsilon)$-error is $\mathcal{\theta}(\frac{V+\ln(1/\delta)}{\epsilon})$, where $V$ is the VC-dimension of the model~\cite{Vapnik:71}. 
This suggests that learning and approximate query answering~\cite{LiL18}  does not require the full  results, and an i.i.d sample can achieve a bounded error. Since this holds for any  model, 
the question to ask is how to sample over the union of joins to enable  a general solution to learning over union. This is the central problem we study in this paper. 

\eat{
an i.i.d sample is a subset of the underlying statistical population of all sources, in which each element has an equal probability of being chosen.
A standard assumption in learning theory is that a training dataset is an i.i.d sample of the underlying distribution~\cite{Vapnik:71}. 
On one hand, most relational sources are not 
stored as single tables due to normalization. Thus, data scientists often perform joins before learning on the join output. 
On the other hand, data scientists often combine   data from multiple sources during data collection. These sources, in turn, may be  described as join paths over internal databases, open data lakes, or web data. 
Because joins are expensive to compute and learning after joins leads to poor training performance due to the introduced 
redundancy avoided by normalization, there has been efforts in 
enabling learning over joins~\cite{SchleichOC16,KumarNP15}, but they are limited to   certain models, including gradient descent with linear regression and cannot be applied to more general models such as SVM. 
Fortunately, an important result from the learning theory states that the sample size needed to train a model up to a $(\delta,\epsilon)$-error is $\mathcal{\theta}(\frac{V+\ln(1/\delta)}{\epsilon})$, where $V$ is the VC-dimension of the model~\cite{Vapnik:71}. 
This suggests that learning does not require the full join results, and an i.i.d sample can achieve a bounded error. Since this holds for any classification model,  sampling over join enables a general solution to learning over joins. In addition, analytics such  estimating COUNT, SUM, AVG, and more advanced tasks such as classification, clustering and regression, can all work with a sample instead of the full data. Sampling over join has been the focus of the data management community due to its connection to query optimization~\cite{sapling-over-join-refs}. These techniques consider the problem of  obtaining a random and independent sample of fixed size from a join path. 
However, when the desired data is collected from distributed sources, 
an i.i.d sample is a subset of the underlying statistical population of all sources, in which each element has an equal probability of being chosen. Nevertheless, if we want to gather information from different paths to perform data-dependent tasks, we have to drop the duplicates that we obtain through different join paths. 
%the sample is required to be an i.i.d sample of the union of data of the sources, where each source is defined with a join path over datasets. 
}



\begin{example} \todo{This  example needs to be shortened and become more concrete, potentially with tables, etc. Ideally, we want example join paths. We would also want paths to contains different datasets.} 
Stores like Walmart may find the patterns for goods that usually being bought by a customer simultaneously, then it can put these goods together so customers would feel convenient or they may be reminded of the related things they have to purchase. In this scenario, Walmart could join the tables to achieve information of goods being bought by each customer.  In real life, customers may go shopping in different Walmart stores, and hence will leave records in different databases. Then in order to analyze the shopping preference of customers, the company can investigate among all the Walmart shops to obtain a more precise result. Instead of performing full join on database of each store and concatenate them together, we could simply sample without performing any join and get the patterns. In this case, we would like to preserve the original distribution of all the record of customers and orders, while significantly reduce the time and space cost compared to sampling after conducting full joins, and thus the problem can be formed as sampling of the disjoint union of multiple joins.
\end{example}

\begin{figure*}
\small
\noindent\begin{minipage}[t]{\textwidth}
    \begin{flalign*}
J1 = &%: (acycic)
{\bf Customer\_W}(CustKey, CName, CNationKey, CAcctBal, \cdots) \bowtie {\bf Part1\_W}(PartKey1, PName1, RetailPrirce1, \cdots) \bowtie &&\\
&{\bf Supplier1\_W}(SuppKey1, SName1, \cdots) \bowtie {\bf PartSupp1\_W}(PartKey1, SuppKey1, AvailQty1, \cdots) \bowtie &&\\
&{\bf Part2\_W}(PartKey2, PName2, RetailPrirce2, \cdots) \bowtie {\bf Supplier2\_W}(SuppKey2, SName2, \cdots) \bowtie &&\\
&{\bf PartSupp2\_W}(PartKey1, SuppKey1, AvailQty1, \cdots) \bowtie {\bf LineItem1\_W}(OrderKey1, PartKey1, SuppKey1, Quantity1, ReturnFlag1, \cdots) \bowtie &&\\
&{\bf Orders1\_W}(OrderKey1, CustKey, OrderStatus1, TotalPrice1, \cdots) \bowtie {\bf Orders2\_W}(OrderKey2, CustKey, OrderStatus2, TotalPrice2, \cdots)  &&\\
&{\bf LineItem2\_W}(OrderKey2, PartKey2, SuppKey2, Quantity2, ReturnFlag2, \cdots) \bowtie 
\end{flalign*}
\begin{flalign*}
J2 = & %: (acyclic)
{\bf Customer\_E}(CustKey, CName, CNationKey, CAcctBal, \cdots) \bowtie {\bf PartSupplier\_E1}(PartKey1, PName1, SuppKey1, SName1, AvailQty1, \cdots) \bowtie &&\\
&{\bf PartSupplier\_E2}(PartKey2, PName2, SuppKey2, SName2, AvailQty2, \cdots) \bowtie &&\\
&{\bf LineItem\_E1}(OrderKey1, PartKey1, SuppKey1, Quantity1, ReturnFlag1, \cdots) \bowtie &&\\
&{\bf DoubleOrders\_E}(OrderKey1, CustKey, OrderStatus1, OrderKey2, OrderStatus2, \cdots) \bowtie &&\\
&{\bf LineItem\_E2}(OrderKey2, PartKey2, SuppKey2, Quantity2, ReturnFlag2, \cdots)  
\end{flalign*}
\begin{flalign*}
J3 = & %: (chain)
{\bf Customer\_MW}(CustKey, CName, CNationKey, CAcctBal, \cdots) \bowtie &&\\
&{\bf DoublePartSupplier\_MW}(PartKey1, SuppKey1, AvailQty1, PartKey2, SuppKey2, AvailQty2, \cdots) \bowtie &&\\
&{\bf DoubleOrdersLineItem\_MW}(CustKey, OrderKey1, PartKey1, SuppKey1, LineNumber1, OrderKey2, PartKey2, SuppKey2, LineNumber2, \cdots) 
\end{flalign*}
    \caption{Example of Union of Joins on Denormalized TPC-H}
    \label{tab:unionexample}
\end{minipage}
\end{figure*}





\eat{
\begin{figure*}
\noindent\begin{minipage}[t]{\textwidth}
    \begin{flalign*}
    J1 = &{\bf Supplier\_W}(Suppkey, Name, Address, NationKey, Phone, AcctBal) \bowtie &&\\
    &{\bf Customer\_W}(CustKey, Name, Address, NationKey, Phone, AcctBal, MktSegment) \bowtie &&\\
    &{\bf Orders\_W}(OrderKey, CustKey, OrderStatus, TotalPrice, OrderDate, OrderPriority, Clerk, ShipPriority)
    \end{flalign*}
    \begin{flalign*}
    J2 = &{\bf Supplier2}(SuppKey, NationKey, Phone, AcctBal) \bowtie {\bf Customer2}(CustKey, Name, Address, NationKey) \bowtie &&\\
    &{\bf Customer3}(Phone, AcctBal, MktSegment) \bowtie {\bf Orders2}(OrderKey, Name, Address) \bowtie &&\\
    &{\bf Orders3}(OrderKey, CustKey, OrderStatus, TotalPrice, OrderDate, OrderPriority, Clerk, ShipPriority)
    \end{flalign*}
    \begin{flalign*}
    J2 = &{\bf Supplier3}(SuppKey, Name, Address, NationKey, Phone, AcctBal) \bowtie &&\\
    &{\bf Customer4}(CUSTKEY, NAME, ADDRESS, NATIONKEY, PHONE, ACCTBAL, MKTSEGMENT) \bowtie &&\\
    &{\bf Orders4}(ORDERKEY, ORDERPRIORITY, CLERK, SHIPPRIORITY) \bowtie &&\\
    &{\bf Orders4}(ORDERKEY, CUSTKEY, ORDERSTATUS, TOTALPRICE, ORDERDATE) 
    \end{flalign*}
    \caption{Example of splitting method}
    \label{tab:unionexample}
\end{minipage}
\end{figure*}
}


\eat{However, as is observed that not all applications need full join, it has been raised that random sampling over join often meets the requirement, which has offered a different angle of reducing cost. Analytical tasks that are fully data-dependent, including estimating COUNT, SUM, AVG, and more advanced tasks such as classification, clustering and regression, can all work with one sample instead of the full data. Among various sample methods, A simple random sample is a subset of the underlying statistical population in which each element has an equal probability of being chosen. Moreover, another important motivation for us is to extend this problem to sampling over multiple join paths instead of just one. Consider the Walmart example again.} 

In this paper, we present a solution for the problem of random sampling over a union of join paths. In particular, we consider two types of union: disjoint union and set union. 

\begin{example} Suppose we would like to estimate the average high school graduation rate for female students in 2022 in each state. To ensure that the study is relatively complete and considers all cities, we use reliable  external sources such as the web and open data to  to obtain information.   However, we only want to keep one tuple of each state, and big cities like NYC, Chicago, etc., could appear more than once. In this scenario, we have to sample over the set union of multiple joins which removes duplicates. 
\end{example}

\eat{
\begin{example} Suppose we would like to estimate the average GDP of countries around the world. To ensure the study is relatively complete and have more countries involved, we rely on reliable  external sources such as the web and open data to  to obtain information from different websites and databases. However, we only want to keep one tuple of each country, and big countries like the US, China, Canada, etc., could appear more than once. In this scenario, we have to sample over the set union of multiple joins which removes duplicates. 
\end{example}}

Given a collection of join paths and sample size $N$, our goal is to ...

In relational algebra and query languages, it is  conventionally  assumed that  {\tt \small union} and  {\tt \small union}  operations can only be executed on queries (join paths) with the same output schema. 
Looser notions of unionability have been considered~\cite{?} that are more applicable to data in the wild, where queries are views over web tables and data lakes~\cite{niffler}. 
We assume all input join paths have the same schema (w.r.t the number and name of attributes) although they may have  different lengths and consist of different datasets. 
If join paths are unionable based on looser notions of unionability, we assume all join path schemas can be unified using a projection operation. 

There are several challenges to address the problem of random sampling over union of joins. 
%Therefore, we aim to propose an algorithm that returns independent and identically distributed samples from multiple join paths and separate the problem into two cases. 

We make the following contributions:
\begin{itemize}
    \item We propose a framework of sampling over disjoint union of multiple chain join paths which could preserve the size and distribution of the samples; we revisit the join size estimation algorithms and employ them in calculating the probability of selecting join paths
    \item We also propose a framework of sampling over set union of multiple chain join paths; we define an innovative method of treating union of joins and give theorems of estimating overlapping information among joins
    \item We revisit strategy group sample algorithm\cite{join_no_index} and extend it to algorithm of sampling over multi-table chain joins without index (in progress); we also propose a hashing approach for sampling which also avoids using index.
\end{itemize}

\fn{data market; union on sets and streams; our joins are not PK-FK}


==> joinsampling.tex <==
\section{Sampling Methods}
\textbf{Estimating Join Size by Correlated Sampling}\\
\textbf{two-table} 
Correlated sampling\cite{cor_sampling} employs hashing method to generate correlated samples which helps handle the join relationship between two tables while sampling. The idea of correlated sampling in two table case is as follows.\\ 
Suppose we want to estimate the size of $J = R_1 \bowtie R_2$ which join on values from the join attribute(s) which is formed as a set $\mathcal{V}$. Let $h:V \rightarrow [0,1]$ be a hash function that uniformly maps the join values into range $[0,1]$. Let $p$ be the sampling probability. Then for every sampled tuple $t_v$ (with value $v$), it's accepted if $h(v) < p$. In this way, a pair of tuples that could be joined share the same join value and thus will both be accepted with probability $p$, and be rejected with probability $1-p$. Let the sample of $R_1$ and $R_2$ be $S_1$ and $S_2$. We can then compute the size of the joined sample and scale it up by $p$, and hence the estimated join size $|\Tilde{J}| = \frac{|S_1 \bowtie S_2|}{p}$.\\
\textbf{multi-table}\\

\noindent \textbf{Estimating Overlap by Sampling with Hashing}
We want to continue to use the hashing and sampling method for join size estimation for overlapping size estimation.\\
General Idea: For $J_1$ and $J_2$, we obtain set of samples when estimating their sizes, say $\Gamma_1 \subset J_1$ and $\Gamma_2 \subset J_2$, where $|\Gamma_1| = |\Gamma_2|$. Let the overlapping part $O_{\Gamma_{12}} = \Gamma_1 \cap \Gamma_2$, then since
$$\frac{|J_1 \cap J_2|}{|J_1| + |J_2|} = \frac{|\Gamma_1 \cap \Gamma_2|}{|\Gamma_1| + |\Gamma_1|}$$
(This is the general idea which is not verified yet. Maybe it's not pluls on the denominater. Need to first guarantee iid, calculate probabilities and variance analysis)
we propose that the estimated pairwise overlapping size between $J_1$ and $J_2$ is
$$O_{12} = |J_1 \cap J_2| = \frac{|O_{\Gamma_{12}}| \cdot (|J_1| + |J_2|)}{|\Gamma_1| + |\Gamma_1|}$$

==> response.tex <==








